Distributional Reinforcement Learning for Multi-Dimensional Reward Functions

A growing trend for value-based reinforcement learning (RL) algorithms is to capture more information than scalar value functions in the value network. One of the most well-known methods in this branch is distributional RL, which models return distribution instead of scalar value. In another line of work, hybrid reward architectures (HRA) in RL have studied to model source-specific value functions for each source of reward, which is also shown to be beneficial in performance. To fully inherit the benefits of distributional RL and hybrid reward architectures, we introduce Multi-Dimensional Distributional DQN (MD3QN), which extends distributional RL to model the joint return distribution from multiple reward sources. As a by-product of joint distribution modeling, MD3QN can capture not only the randomness in returns for each source of reward, but also the rich reward correlation between the randomness of different sources. We prove the convergence for the joint distributional Bellman operator and build our empirical algorithm by minimizing the Maximum Mean Discrepancy between joint return distribution and its Bellman target. In experiments, our method accurately models the joint return distribution in environments with richly correlated reward functions, and outperforms previous RL methods utilizing multi-dimensional reward functions in the control setting.

==> Distributional RL with Multiple Reward/src/1-intro.tex <==
\section{Introduction}


% para #1: key point in value-based RL: interpretation of value estimates

Making value network capture more information than scalar value functions is a growing trend in value-based reinforcement learning, which helps the agent gain more knowledge about the environment and has great potentials to improve the sample efficiency %ability 
of RL agents. 
In the early stage %At the starting stage 
of deep reinforcement learning, DQN~\citep{mnih2013playing} uses the scalar output of the neural network to represent value functions. As value-based RL algorithms evolve, distributional RL algorithms start to use neural networks to approximate return distributions for each state-action pair, and take action based on the expectation of return distributions. 
By capturing the randomness in return as auxiliary tasks, distributional RL agents can gain more knowledge about the environment and learn better representations to avoid state aliasing~\citep{bellemare2017distributional}.
Distributional RL algorithms including C51~\citep{bellemare2017distributional}, QR-DQN~\citep{dabney2018distributional}, IQN~\citep{dabney2018implicit},  FQF~\citep{FQF} and MMDQN~\citep{nguyen2020distributional}  achieve substantial performance gain compared to DQN. 

% para #2: hybrid reward value outputs, and why they are effective


In another line of work, HRA~\citep{van2017hybrid} and RD$^2$~\citep{lin2020rd} consider the setting where multiple sources of reward exist in the environment and modify the value network to model source-specific value function for each source of reward. In these works, the outputs of value networks can be interpreted as multiple source-specific value functions, and the agent takes action based on the sum of all source-specific value functions. Similar to return distribution, estimating the source-specific value functions can be seen as auxiliary tasks, which serve as additional supervision for how the total reward is composed and enable the agent to learn better representations. 
Several previous works support that it is beneficial to model source-specific value functions~\citep{boutilier1995exploiting, sutton2011horde, van2017hybrid, lin2020rd}. 


%On another aspect, HRA~\citep{van2017hybrid} and \textcolor{blue}{RD$^2$}~\citep{lin2020rd} consider the setting where multiple reward sources exist in the environment and modify the value network to estimate source-specific value \textcolor{blue}{functions}. In \textcolor{blue}{this} branch of \textcolor{blue}{works}, the outputs of value network can be interpreted as multiple source-specific value \textcolor{blue}{functions}, and agent takes action based on the sum of all source-specific value \textcolor{blue}{functions}. Many evidences support that it is beneficial to learn source-specific value functions, instead of learning the value function for the mixture of reward sources. \textcolor{blue}{Intuitively}, the source-specific return serves as additional supervision for how the total reward is composed, which strengthen the generalization capabilities of the value function. Empirically, experimental studies in HRA and RD$^2$ support that learning source-specific value \textcolor{blue}{functions} can get better performance. Additionally, it is common in RL where multiple \textcolor{blue}{sources} of reward \textcolor{blue}{exists} in one environment. Other existing \textcolor{blue}{works}, like Factored MDP \citep{boutilier1995exploiting} and Horde \citep{sutton2011horde}, also consider the same settings and model source-specific value \textcolor{blue}{functions}. \textcolor{red}{缩写一下}


% para #3: our work

Towards providing more supervision signals and enabling agents to gain more knowledge about the environment, we propose to capture the correlated randomness in source-specific returns. Specifically, we consider the source-specific returns from all sources of rewards as a multi-dimensional random variable, and capture its joint distribution to model the randomness of returns from different sources. This provides an informative learning target for our agent. % Our method, Multi-Dimensional Distributional DQN (MDDQN), builds the framework to capture correlated randomness with joint distribution. 
The framework is general and can be extended to capture the correlated randomness of other types of random variables than rewards. For example, we can capture the correlation between achieving different goals in goal-conditioned reinforcement learning~\citep{schaul2015universal}, or visiting different states in successor representation~\citep{kulkarni2016deep}. In this paper, we focus on the method for learning joint return distribution of given source-specific rewards and leave the extension to more general settings for future work. 

%In our work, we propose Hybrid Reward distributional RL for modeling \textcolor{blue}{the joint value distribution} which fully inherit the benefits of distributional RL and leveraging hybrid-source rewards. Our algorithm framework recognizes future hybrid-source returns as a high-dimensional random variable, and the value network directly outputs the distribution of this high dimensional variable. We build a highly general and informative value network \textcolor{blue}{for the joint value distribution, which can} accurately reconstruct (1) the value distribution from each reward source and (2) the value distribution of total reward. Beyond, the joint distribution modeling enable the agent to infer about the correlation between each reward source. 

Following existing works on distributional RL, we study the convergence of the Bellman operator and propose an empirical algorithm to approximate the Bellman operator. First, we define the joint distributional Bellman operator, and prove its convergence under the Wasserstein metric. % We point out a questionable claim in existing works of distributional RL, and argue that we can use other metrics than the Wasserstein metric over joint distribution as training losses to approximate the Bellman operator. 
To derive an empirical algorithm, our proposed method (MD3QN) approximates the joint distributional Bellman operator by minimizing the Maximum Mean Discrepancy~(MMD) loss over joint return distributions and its Bellman target. MMD holds desirable properties that, it is a metric over joint distribution and its square can be unbiasedly optimized with batch samples. This enables our algorithm to approximate the Bellman operator accurately when the number of samples goes to infinity and the loss is minimized to zero. 
%This prevents MDDQN from learning a biased training signal, which is not guaranteed if we apply other distributional metric. 
% To deal with the different scale for rewards from different sources, we further propose to use reweighted norm with adaptive weight in the kernels of MMD to balance different rewards.
%We also propose a simple temporal difference loss based on transition samples, which is the joint distributional metric between current step and next step, and can be optimized unbiasedly. Our theory provides guarantees for convergence on the modeling of high-dimensional joint distribution when the temporal difference loss is effectively optimized. 
In experiments on Atari games and other environments with pixel inputs, our method accurately models the multi-dimensional joint distribution from multiple sources of reward. %which encodes the information about value distribution and reward source correlation. 
Moreover, our algorithm outperforms previous work HRA which also separately models multiple sources of reward on Atari game environments. %, and meanwhile outperform existing distributional RL algorithms including IQN and MMDQN.

Our contributions can be summarized as follows: 
\begin{itemize}
    \item We propose a distributional RL algorithm, MD3QN, that extends distributional RL algorithms to model the joint return distribution from multiple sources of reward.
    %Our proposed method is the first distributional RL algorithm that learns a high-dimensional joint distribution model by temporal difference loss. Our representation is informative enough to accurately encodes value distribution and specific-source reward information. 
    \item We establish convergence results for the joint distributional Bellman operator, and our proposed algorithm MD3QN approximates this Bellman operator by minimizing MMD loss over joint return distribution and its Bellman target. 
    %We provide theoretical \textcolor{blue}{guarantees for the convergence of joint distributional bellman operator.} \textcolor{red}{Revise this sentence.} %that the algorithm converge to the ground truth high-dimensional joint distribution when the temporal difference loss is effectively optimized. 
   % \item \textcolor{blue}{We propose adapting re-weighted kernel for MMD loss over high-dimensional value distributions, in order to deal with the different scale of hybrid sources of reward. }\textcolor{red}{Revise this sentence.}
    \item Empirically, our method outperforms previous RL algorithms utilizing multiple sources of reward, and accurately models the joint return distribution from all sources of rewards. 
\end{itemize}

%The rest of our paper will be formed as follows: in section 2 we will describe background about distributional RL and HRA; in section 3 we will describe our method (HRDRL) in detail; in section 4 we will introduce related work to our \textcolor{blue}{method}; in section 5 we will illustrate all experimental results; in section 6 we will conclude the novelty and contribution of our work and \textcolor{blue}{discuss} future work direction. 

==> Distributional RL with Multiple Reward/src/2-related-work.tex <==
\section{Related Work}

% ATTENTION: some phrases need to be modified

% para 1: RL + distributional RL algorithm 

%C51 \citep{bellemare2017distributional} shows that the distribution of the random returns, whose expectation constitutes the aforementioned value, can be described by the distributional analogue of Bellman’s equation. C51 uses fixed number of bins with fixed range, and model the probability of future returns that belongs to each bins. QR-DQN \citep{dabney2018distributional} propose an alternate pair of choices, parameterizing the distribution by a uniform mixture of Diracs whose locations are adjusted using quantile regression. IQN \citep{dabney2018implicit} uses quantile values as neural network's input to approximate quantile function, which is capable of approximating any distribution over returns given sufficient network capacity. This series of work mainly focus on parameterization of value distributions. MMDQN \citep{nguyen2020distributional} mainly focus on the MMD loss function applied to minimize distributional metric. The sample-based MMD metric enable MMDQN to be trained on arbitrary sample-based distribution parameterization. 

Distributional RL algorithms propose to model the entire distribution, rather than the expectation, of the random variable return. C51~\citep{bellemare2017distributional} is the first distributional RL algorithm, and establishes the convergence of distributional RL algorithms based on the contraction property of the distributional Bellman operator. To approximate such an operator with sample transitions, different distributional algorithms employ different losses over distribution, along with different parameterization for distribution. C51 uses KL-divergence as loss and categorical distribution as parameterization. QR-DQN~\citep{dabney2018distributional} takes quantile regression as surrogate loss for the Wasserstein metric, and approximates a set of quantile values with fixed probabilities. IQN~\citep{dabney2018implicit} and FQF~\citep{FQF} extend QR-DQN to learn with sampled probabilities and self-adjusted probabilities. The current SOTA method in distributional RL is MMDQN~\citep{nguyen2020distributional}, which takes MMD loss with a non-parametric approach by modeling deterministic samples from return distribution. Our method extends the theoretical work of C51, and the empirical algorithm of MMDQN to multi-dimensional returns. While distributional RL algorithms focus on capturing the randomness in return, our method first proposes to capture the correlation between different randomness from different reward sources.

% para 3: HRA

HRA~\citep{van2017hybrid} proposes a hybrid architecture to separately model the value functions for different sources of rewards. %Although the original work of HRA claims that HRA can tackle the difficulty of value function generalization in RL, they do not provide empirical justification for their claim. Compared to their work, we compare the performance between HRA and DQN on Atari games, and empirically prove that hybrid architecture can help modeling hybrid-source returns.
Their work provides empirical justification that learning with hybrid rewards can improve sample efficiency. 
HRA is built upon the Horde architecture~\citep{Horde}, which trains a separate general value function (GVF) for each pseudo-reward function. The Horde architecture uses a large number of GVFs to model general knowledge about the environment.
Previous works on reward decomposition also demonstrate that it is beneficial to learn with multiple reward functions~\citep{lin2020rd}. 
Based on HRA, our method further considers the correlated randomness in hybrid-source returns with a joint distribution model. 
%We also consider the different scale of rewards from hybrid sources, which is ignored in HRA. 
%Our proposed method further models distributional information for future values while maintaining the hybrid architecture, which extends the high performance of distributional RL without suffering from issues of hybrid-source and hybrid-scale rewards. % RDRD \citep{lin2020rd} ... . 

Bellman GAN~\citep{freirich2019distributional} shows that distributional RL can be used for multi-dimensional rewards. Compared to this work, we additionally provide the theoretical convergence results for the joint distributional Bellman operator, an algorithm where the gradient of objective function~(MMD) can be unbiasedly estimated, and experimental results that directly compare the modeled joint distribution to the true distribution, demonstrating the accuracy of our method under diverse reward correlations. DRDRL~\citep{lin2019distributional} focuses on decomposing multiple types of rewards from one source reward, while in our paper, we are directly provided with multiple types of rewards as inputs, and model the joint distribution of different sources of rewards.

By modeling the joint return distribution, we provide an informative target to learn, which can be seen as auxiliary tasks. Previous works in RL have constructed various auxiliary tasks to learn better representations, such as methods based on temporal structures~\citep{aytar2018playing} and local spatial structures~\citep{anand2019unsupervised}.  Compared with these methods, our method does not entirely focus on learning better state representations. The learned joint distribution is also beneficial to risk-sensitive tasks~\citep{zhang2020cautious}. Besides, our method for learning the joint distribution of multi-dimensional random variables is general, and can be further combined with goal-conditioned RL~\citep{schaul2015universal} or successor representation~\citep{kulkarni2016deep} to capture correlated randomness in achieving different goals or visiting different states. 



%\textcolor{red}{goal conditional, successor feature, state aliasing, state representation learning}

% para 2: reward clipping, and how to handle reward clipping

\iffalse
Reward clipping is a commonly used heuristics, which starts to be used in DQN paper \citep{mnih2013playing}. Almost all subsequent state-of-the-art RL algorithm on Atari environment uses reward clipping setting, including C51, IQN and MMDQN. PopArt \citep{hessel2019multi} prevents the use of reward clipping by performing adaptive normalization on the return estimation, and define the temporal difference error on the normalized space. One of previous work \citep{hessel2019inductive} analyzes the effect of reward clipping on Atari games, and shows that the performance of RL agents significantly degrade when reward clipping is not performed. \textcolor{blue}{We borrow the idea of adaptive normalization and integrate it with MMD metric. Our method will not change the optimal solution as long as the kernel in MMD is characteristic.}
\fi

% para 4: 

==> Distributional RL with Multiple Reward/src/3-background.tex <==
\section{Background}

\subsection{Notations and Problem Setting}

Since our work considers multiple sources of reward exist in the environment, our problem setting %has subtle difference compared with 
is slightly different from the traditional RL setting in reward function. We consider a Markov Decision Process with multiple sources of reward defined by $(\mathcal{S},\mathcal{A},P,\bm{R},\rho_0,\gamma)$, where $\mathcal{S}$ is the set of states, $\mathcal{A}$ is the finite set of actions, $P: \mathcal{S} \times \mathcal{A} \rightarrow \mathcal{P}(\mathcal{S})$ denotes the transition probability, $\bm{R} : \mathcal{S} \times \mathcal{A} \rightarrow \mathcal{P}(\mathbb{R}^N)$ denotes the reward function for a total of $N$ sources of reward, $\rho_0 : \mathcal{P}(\mathcal{S})$ denotes the distribution of initial state $S_0$, $\gamma \in (0,1)$ is the discount factor. Given a policy $\pi: \mathcal{S} \rightarrow \mathcal{P}(\mathcal{A})$, a trajectory is generated by $s_0 \sim \rho_0$, $a_t \sim \pi(s_t)$, $s_{t+1} \sim P(s_t, a_t)$ and $\bm{r}_{t} = [r_{t, 1}, r_{t, 2},..., r_{t, N}]^\top \sim \bm{R}(s_t, a_t)$. 
We use $r_t = \sum_{n=1}^{N}r_{t, n}$ to denote the total reward received at time $t$. 
%We use $\vec{r}_t$ to denote the reward vector received at time $t$,  $r_{t, k}$ to denote the reward received at time $t$ from $k$-th reward source, and $r_t = \sum_{k=1}^{K}r_{t, k}$ to denote the total reward received at time $t$. 
The goal for reinforcement learning algorithms is to find the optimal policy $\pi$ which maximizes the expected total return from all sources, given by $J(\pi) = \mathbb{E}_\pi[\sum_{t=0}^{\infty}\gamma^t \sum_{n=1}^N r_{t,n}]$. 

Next we describe value-based reinforcement learning algorithms in a general framework. In DQN, the value network $Q(s,a;\theta)$ captures the scalar value function, where $\theta$ is the parameters of the value network. $\theta_0$ is the initial value of $\theta$. In $i$-th iteration, the training objective for $\theta_i$ is\footnote{In practical implementations, the iterative process is approximated by substituting $\theta_{i-1}$ by the parameter of the target network which tracks the exponential moving average of the online network parameters $\theta_{i}$. }
\begin{align}
    L(\theta_i) &= \mathbb{E}_{s_t,a_t,r_t,s_{s+1}} [(Q(s_t,a_t;\theta_i) - y_i)^2], \\
    \text{ where } y_i &= r_t + \gamma \max_{a'} Q(s_{t+1}, a';\theta_{i-1}),
\end{align}
and $s_t,a_t,r_t,s_{t+1}$ are sampled from the replay memory. 

\subsection{Distributional RL}

%In C51, IQN, MMDQN and other distributional RL algorithm, 
In distributional RL algorithms such as C51, IQN and MMD-DQN, 
$\mu(s,a;\theta)$ captures the return distribution for each state action pair $(s, a)$. In $i$-th iteration, the training objective for $\theta_i$ is
\begin{align}
    L(\theta_i) &= \mathbb{E}_{s_t,a_t,\bm{r}_t,s_{t+1}} [d(\mu(s_t,a_t;\theta_i), \eta_i)], \\
    \text{ where } \eta_i &= \left(f_{r_t,\gamma}\right)_{\#} \mu(s_{t+1}, a';\theta_{i-1}), a' = \argmax_{a}\mathbb{E}_{Z \sim \mu(s_{t+1}, a;\theta_{i-1})}[Z].
\end{align}

Here $f_{r,\gamma}(x):=r + \gamma \cdot x$. Given a probability distribution $\nu \in \mathcal{P}(\mathbb{R})$, $f_{\#}\nu \in \mathcal{P}(\mathbb{R})$ is the pushforward measure defined by $f_{\#}\nu(A)=\nu(f^{-1}(A))$ for all Borel sets $A\subseteq \mathbb{R}$ and a measurable function $f:\mathbb{R} \rightarrow \mathbb{R}$ \citep{rowland2018analysis}.
$d$ is some distributional metric different in each method. In C51 $d$ is KL divergence, in MMDQN $d$ is Maximum Mean Discrepancy, while in QR-DQN and IQN $d$ is Wasserstein metric, which is optimized approximately via quantile regression loss. 

\subsection{Hybrid Reward Architecture}
%\textcolor{blue}{we use $Q$ to denote the vectored value function, and $Q_k$ denoting the $k$-th value function with respect to the $k$-th reward. }
HRA \citep{van2017hybrid} proposes the hybrid architecture to separately model the value function for each source of reward. With multiple sources of reward, 
%we use $\bm{r} \in \mathbb{R}^K$ to denote the reward vector, $r_k \in \mathbb{R}$ to denote the reward from the $k$-th source, and $r \in \mathbb{R}$  to denote the sum over different reward sources. 
we use $\bm{Q}: (\mathbb{R}^N)^{\mathcal{S} \times \mathcal{A}}$ and $Q_n: \mathbb{R}^{\mathcal{S} \times \mathcal{A}}$ to denote the vectored value function and the $n$-th value function respectively. 

The loss used by HRA is given by: 
\begin{align}
    L(\theta_i) &= \mathbb{E}_{s_t,a_t,\bm{r}_t,s_{t+1}} [\|\bm{Q}(s_t,a_t;\theta_i)- \bm{y}_i\|_2^2], \\
    %L(\theta_i) &= \mathbb{E}_{s,a,r,s'} [\sum_{k = 1}^{K}(Q_k(s,a;\theta_i)- y_{i,k})^2] \\
    \text{ where } y_{i,n} &= r_{t,n} + \gamma Q_n(s_{t+1}, a';\theta_{i-1}), a' = \argmax_{a}Q_n(s_{t+1}, a;\theta_{i-1}).
\end{align}

RD$^2$ \citep{lin2020rd} uses the similar hybrid architecture, which also learns the value function separately for each source of reward, but with slight differences with HRA in how the next action $a'$ is computed. The loss used by RD$^2$ is given by\footnote{In equation \eqref{eq-8}, $\bm{y}_i$ is an N-dimensional vector. We use the bold font to denote that the variable is for the multi-dimensional reward function. }
\begin{align}
    L(\theta_i) &= \mathbb{E}_{s_t,a_t,\bm{r}_t,s_{t+1}} [\|\bm{Q}(s_t,a_t;\theta_i)- \bm{y}_i\|_2^2], \\
    \text{ where } \bm{y}_i &= \bm{r} + \gamma \bm{Q}(s_{t+1}, a';\theta_{i-1}), a' = \argmax_{a}\sum_{n=1}^{N}Q_n(s_{t+1}, a;\theta_{i-1}). \label{eq-8}
\end{align}


==> Distributional RL with Multiple Reward/src/5-method-notation.tex <==

\section{Distributional Reinforcement Learning for Multi-Dimensional Reward Functions}

In this paper, we propose to capture the correlated randomness from multiple sources of reward, forcing the agent to gain more knowledge about the environment and learn better representations. Specifically, we consider the joint distribution of returns from different sources of reward. 
First, we introduce the joint distributional Bellman operator and establish its convergence. % We point out a questionable claim in existing work~\citep{bellemare2017distributional,nguyen2020distributional}, that we must use the same metric for proving convergence and as training loss. We illustrate that, once the convergence of the Bellman operator is proved under a certain metric, we can use other metrics than the metric for proving convergence, as training loss to approximate the Bellman operator. 
Second, we introduce an empirical algorithm, which approximates the joint distributional Bellman operator through stochastic optimization with deep neural networks. Inspired by MMDQN~\citep{nguyen2020distributional}, we introduce a temporal difference loss based on Maximum Mean Discrepancy over joint return distributions.
Finally, we present full implementation details of our method, including network architectures and algorithms. % In order to adapt to multiple reward sources with different reward scale, we also introduce re-weighted norm with adaptive weight for gaussian kernels in the MMD loss to balance between rewards from different sources.

%\textcolor{blue}{In this paper, we consider the joint return distribution under the hybrid reward setting. First, we introduce the joint distributional bellman operator and establish its convergence. To approximate such operator through stochastic optimization in practical algorithm with deep neural networks, we then introduce a temporal difference loss based on Maximum Mean Discrepancy over joint return distributions, as inspired by \cite{}. Finally we give full implementation details of our method, including network architectures and loss computations. }

%\textcolor{red}{Both the theoretical and algorithmic parts of our method can be seen as extensions of existing theoretical and algorithmic works on 1-dimension to K-dimension. It is worth mentioning that such extension is non-trivial, in that we fix some issues and make some adaptations to K-dimension. We find the 1-dimensional contraction proof in \cite{C51} skip some steps, making it hard to follow, therefore we give a more detailed contraction proof under the joint distribution setting. While the original algorithm in 1-dimension takes use of deterministic samples from return distribution, we propose to estimate stochastic samples with more flexibility to approximate the whole return distribution as the number of samples approach infinite. In order to deal with different scale of reward from hybrid sources, we also introduce re-weighted norm for gaussian kernels in the MMD loss. }


%We first define the hybird-source return as a K-dimensional random variable, and introduce Wasserstein metric $Wp$ the joint distribution and  on the settings and establish the convergence of the joint distributional bellman operator. 


%In this section, we firstly focus on the settings and convergence analysis for learning the joint value distribution of hybrid-source return. We prove that iteratively \textcolor{blue}{applying} %adapting by 
%joint distributional Bellman operator will make the estimation converge to the ground truth value distribution. 
%We then introduce a temporal difference error based on metric over joint value distribution, and explain why optimizing the loss can be approximated as applying joint distributional Bellman operator. 
%Finally we give full implementation details of our method, including network architectures and loss computations. 


\subsection{Definitions and Settings}

%We define $\vec{Z}^\pi(s,a)$ as
We consider the joint return under policy $\pi$ as a random vector $\bm{Z}^\pi(s,a)$ composed of $N$ random variables $\bm{Z}^\pi(s,a) = \left( Z^\pi_1(s,a), \cdots, Z^\pi_N(s,a) \right)^\top$:
\begin{align}
    \bm{Z}^\pi(s,a) &= \sum_{t=0}^\infty \gamma^t \bm{r}_t, \\
    \text{ where } s_0 &= s, a_0 = a, \bm{r}_t \sim R(\cdot|s_t, a_t), s_{t+1} \sim P(\cdot|s_t, a_t), a_{t+1} \sim \pi(\cdot|s_{t+1}).
\end{align}

%We can interpret $\vec{Z}^\pi(s,a)$ as the joint distribution for the discounted return of multiple source reward. 
Here $Z^\pi_i(s,a)$ denotes the $i$-th dimension of $\bm{Z}^\pi(s,a)$, which is the random variable of the $i$-th source of discounted return. Here the random variables of discounted return in different sources can be correlated. 
%We use $\bm{Z}: \mathcal{S} \times \mathcal{A} \rightarrow \mathcal{P}(\mathbb{R}^K)$ to denote a joint return distribution model, where $\bm{Z}(s,a) \in \mathcal{P}(\mathbb{R}^K)$ is the joint distribution predicted by the model on state action pair $(s,a)$ of future returns over multiple reward sources.
We denote the distribution of $\bm{Z}^\pi$ as $\bm{\mu}^{\pi} = \text{Law} \left( \bm{Z}^\pi \right)$, and the distribution of $i$-th random variable $Z^\pi_i$ as $\mu_i^{\pi} = \text{Law} \left( Z^\pi_{i} \right)$, where $\bm{\mu}^{\pi} \in \mathcal{P}(\mathbb{R}^N)^{\mathcal{S} \times \mathcal{A}}$ and $\mu_i^{\pi} \in \mathcal{P}(\mathbb{R})^{\mathcal{S} \times \mathcal{A}}$.
We let $\bm{\mu} \in \mathcal{P}(\mathbb{R}^N)^{\mathcal{S} \times \mathcal{A}}$ to denote arbitrary joint distribution over all state-action pairs,
%distributional model,
and the goal of our algorithm is to let the joint distribution $\bm{\mu}$ to be as close to the joint distribution $\bm{\mu}^{\pi}$ as possible in policy evaluation setting, i.e. to model the real joint return distribution. % \textcolor{blue}{What about control setting?}

To measure how close two $N$-dimensional joint distributions are, we adopt the Wasserstein metric $W_p$.  %If we have 
For two joint distributions $\nu_1, \nu_2 \in \mathcal{P}(\mathbb{R}^N)$, the p-Wasserstein metric $W_p(\nu_1, \nu_2)$ on Euclidean distance $d$ is given by: 
\begin{equation}
    W_p(\nu_1, \nu_2) = \left(\inf_{f \in \Gamma(\nu_1, \nu_2)} \int_{\mathbb{R}^N \times \mathbb{R}^N} d(x, y)^p f(x,y) d^N x d^N y \right)^{1/p},
    %W_p(\mu, \nu) = \left(\inf_{f \in \Gamma(\mu, \nu)} \int_{\mathbb{R}^K \times \mathbb{R}^K} d(x, y)^p  \mathrm{d} f(x,y) \right)^{1/p}
\end{equation}
where $\Gamma(\nu_1, \nu_2)$ is the collection of all distributions with marginal distributions $\nu_1$ and $\nu_2$ on the first and second $N$ random variables %factors 
respectively. The Wasserstein distance can be interpreted as the minimum moving distance to move all the mass from distribution $\nu_1$ to distribution $\nu_2$. 

We further define the supremum-$p$-Wasserstein distance on $\mathcal{P}(\mathbb{R}^N)^{\mathcal{S} \times \mathcal{A}}$ by
\begin{equation}
    %d_p(W_1, W_2) := \max_{s,a} W_p(W_1(s,a), W_2(s,a)). 
\bar{d}_p(\bm{\mu}_1, \bm{\mu}_2) := \sup_{s,a} W_p(\bm{\mu}_1(s,a), \bm{\mu}_2(s,a)),
\end{equation}
where $\bm{\mu}_1, \bm{\mu}_2 \in \mathcal{P}(\mathbb{R}^N)^{\mathcal{S} \times \mathcal{A}}$.

We will use $\bar{d}_p$ to establish the convergence of the joint distributional Bellman operator. 
\iffalse
\begin{lemma}
    $\bar{d}_p$ is a metric over joint return distributions.
\end{lemma}
\fi

\subsection{Convergence of the Joint Distributional Bellman Operator}
%\textcolor{blue}{We extend the theoretical results on distributional bellman operator from 1-dimension distribution in C51, to high-dimensional distribution in our case. It is worth mentioning that it is non-trivial to extend the theoretical results to high-dimensional distribution, where the wasserstein distance does not have nice formulation as in 1-dimensional case. Detailed proofs can be found in Appendix.  }
%The theory framework is mainly based on C51 paper \citep{bellemare2017distributional}, but our conclusion is the extension of theirs and require more work than C51. 
We define the joint distributional Bellman evaluation operator $\mathcal{T}^\pi$ as
\begin{align}
    \mathcal{T}^\pi \bm{\mu}(s_t,a_t) &\stackrel{D}{\coloneqq} \int_{\mathcal{S}} \int_{\mathcal{A}} \int_{\mathbb{R} ^ N} (f_{\bm{r}_t, \gamma})_{\#} \bm{\mu}(s_{t+1}, a_{t+1}) R(d\bm{r}_t|s_t,a_t) \pi(da_{t+1}|s_{t+1}) P(ds_{t+1}|s_t,a_t),
\end{align}
where $f_{\bm{r}, \gamma}(\bm{x}) = \bm{r} + \gamma \bm{x}$, where $\bm{x}, \bm{r} \in \mathbb{R}^N$ and $f_{\#} \bm{\mu}$ is the pushforward measure which is a $N$-dimensional extension of the pushforward measure defined in \cite{rowland2018analysis}.
The below theorem shows that $\mathcal{T}^\pi$ is a $\gamma$-contraction operator on $\bar{d}_p$. % We provide detailed proof of Theorem 1 in Appendix A. 
\begin{theorem}
    %For two joint distribution models
    For two joint distributions $\bm{\mu}_1$ and $\bm{\mu}_2$, %$W_1$ and $W_2$, 
    we have
    \begin{equation}
        %d_p(\mathcal{T}^\pi W_1, \mathcal{T}^\pi W_2) \leq \gamma d_p(W_1, W_2)
        \bar{d}_p(\mathcal{T}^\pi \bm{\mu}_1, \mathcal{T}^\pi \bm{\mu}_2) \leq \gamma \bar{d}_p(\bm{\mu}_1, \bm{\mu}_2).
    \end{equation}
\end{theorem}

The proof for Theorem 1 is provided in Appendix A.1 which can be briefly described as follows. In Lemma 3, we prove that if the Wasserstein distance of two joint distributions is $C$, then after applying the same linear transformation to these two distributions with a scale factor of $\gamma$, the Wasserstein distance is at most $\gamma C$. In Lemma 4, we prove that the Wasserstein distance of two joint distributions under the same conditional random variable $A$ is no greater than the maximum Wasserstein distance over all possible conditions $A=a$. By Lemma 3 and Lemma 4, we are able to prove the contraction results in Theorem 1. 

Following the result of Theorem 1, we consider the following scenario: initially we have a joint distribution $\bm{\mu}_0 \in \mathcal{P}(\mathbb{R}^N)^{\mathcal{S} \times \mathcal{A}}$ over all state-action pairs, and by iteratively applying the Bellman evaluation operator, we get $\bm{\mu}_{i+1} = \mathcal{T}^\pi \bm{\mu}_i $.
According to Banach's fixed point theorem, operator $\mathcal{T}^\pi$ has a unique fixed point, which is $\bm{\mu}^\pi$ by definition. 
%Since $\bm{Z}^\pi$ is the fix point of operator $\mathcal{T}^\pi$, 
The distance between $\bm{\mu}_i$ and $\bm{\mu}^\pi$ decays as $i$ increases. We have the following corollary:
\begin{corollary}
    If $\bm{\mu}_{i+1} = \mathcal{T}^\pi \bm{\mu}_i $, then as $i \rightarrow \infty$, $\bm{\mu}_i \rightarrow \bm{\mu}^\pi$. 
\end{corollary}
We also provide contraction proof on the expectation of the optimality operator.
%%%%%% \blue{Please check here}
The joint distributional Bellman optimality operator $\mathcal{T}$ is defined as
\begin{align}
    \mathcal{T}\bm{\mu}(s_t,a_t) &\stackrel{D}{\coloneqq} \int_{\mathcal{S}} \int_{\mathbb{R} ^ N} (f_{\bm{r}_t,\gamma})_{\#} \bm{\mu}(s_{t+1}, a') R(d\bm{r}_t|s_t,a_t) P(ds_{t+1}|s_t,a_t), \label{eq-optimal-op} \\
    \text{ where } & a' \in \argmax_{a} \mathbb{E}_{\bm{Z} \sim \bm{\mu}(s_{t+1}, a)} \sum_{n=1}^N Z_n \text{ and } Z_n \text{ is the  }n\text{-th element in } \bm{Z}. \label{eq-optimal-op-where}
\end{align}

\begin{theorem}
    %For two joint distribution models
    For two joint distributions $\bm{\mu}_1$ and $\bm{\mu}_2$, %$W_1$ and $W_2$, 
    we have
    \begin{equation}
        %\vert \vert \mathbb{E} \mathcal{T} W_1 - \mathbb{E} \mathcal{T} W_2 \vert \vert_{\infty} \leq \gamma \vert \vert \mathbb{E}  W_1 - \mathbb{E} W_2 \vert \vert
        \vert \vert (\mathbb{E}_{\sum}) (\mathcal{T} \bm{\mu}_1) - (\mathbb{E}_{\sum}) (\mathcal{T} \bm{\mu}_2) \vert \vert_{\infty} \leq \gamma \vert \vert (\mathbb{E}_{\sum})\bm{\mu}_{1} - (\mathbb{E}_{\sum})\bm{\mu}_{2} \vert \vert_{\infty},
    \end{equation}
\end{theorem}
%\textcolor{red}{redefine the expectation here! Should be sum over all sub-returns. } where \textcolor{red}{$\mu_{\cdot,k}$} represents the marginal distribution for the $k$-th source-specific return.
where the operator $\mathbb{E}_{\sum}$ is defined by $ \left( \mathbb{E}_{\sum} \right) \bm{\mu}(s,a) = \mathbb{E}_{\bm{Z} \sim \bm{\mu}(s,a)} \sum_{n=1}^N Z_n$ for any $(s,a)$, and $Z_n$ is the $n$-th element in $\bm{Z}$. The operator $\mathbb{E}_{\sum}$ converts the joint distribution over all state-action pairs to the corresponding total expected returns over all state-action pairs.  
%%%%%%

\begin{corollary}
    If $\bm{\mu}_{i+1} = \mathcal{T} \bm{\mu}_i $, then as $i \rightarrow \infty$, $\mathbb{E}_{\bm{Z} \sim \bm{\mu}_i(s,a)} \sum_{n=1}^N Z_n \rightarrow Q^*(s,a)$ for all $(s,a)$.%\mathbb{E}[\sum_{k=1}^{K} Z^{*}_{i,k}]$. 
\end{corollary}

%The
Corollary 2 can be interpreted as follows: as we iteratively apply the joint distributional Bellman optimality operator, the expected total return of the joint distribution $\bm{\mu}_i$ will converge to optimal value function. We refer the readers to Appendix A.1 for detailed proofs for all the lemmas, theorems, and corollaries.


%There is a common misunderstanding in existing work that it is necessary to use the same metric to prove convergence and as training loss~\citep{bellemare2017distributional, nguyen2020distributional}. However, we argue that, convergence is the property of the operator itself, regardless of the metric. If the operator is proved to be contraction under one metric, then applying the operator iteratively will lead to convergence to a fixed point. In contrast, training loss is used to "apply" the operator. In fact, we can use any loss, as long as we can guarantee the distribution and its Bellman target are identical when the loss is minimized. 
%For example, in C51~\citep{bellemare2017distributional}, the Cramer distance is used implicitly in the projection step, and the projected operator is proved to be contraction under cramer distance. Then, we can apply this projected operator with KL-divergence, since KL-divengence is minimized if and only if two distributions are identical. \textcolor{red}{maybe we need to week the claim}

Next, we establish the empirical algorithm which simulates the iterative process in Corollary 1 and Corollary 2 with a neural network approximating the joint distribution $\bm{\mu}_{i}$ for all state-action pairs. 

\iffalse
There is a questionable claim in existing work that we must use the same metric to prove convergence and as training loss~\citep{bellemare2017distributional, nguyen2020distributional}. We clarify that the metric for proving convergence and the metric for training play different roles, and are not necessarily the same metric. 
For example, supremum Cramer distance is used to prove the contraction property of the projected Bellman operator in C51~\citep{pmlr-v84-rowland18a}, while KL-divergence is used to approximate the projected operator in C51~\citep{bellemare2017distributional} and is used as training loss. With infinite sampled transitions and an enough expressive value networks, C51 can approximate the projected Bellman operator exactly when the KL-divergence of modeled distribution and its Bellman target is minimized to zero. This may partially explain why replacing KL-divergence with Cramer loss does not lead to improvement in performance~\citep{pmlr-v89-bellemare19a}.
\fi


\subsection{Optimizing MMD as Approximation for Bellman Operator}

%\textcolor{blue}{1. We extend existing distribution RL algorithm to high-dimensional? or we approximate the joint distributional bellman operator with xxx loss? 2. C51 is not easy to scale to high-dimensional. Sample-based method is much better.3. approximate continuous distribution with samples. logic is not clear yet. Try to figure out a good logic tomorrow. }

In practical algorithms, the joint distribution $\bm{\mu}_i(s,a)$ is represented by deep neural network $\bm{\mu}(s,a;\theta_{i})$ which outputs joint distribution for each state-action pair with parameter $\theta_i$. In the $(i+1)$-th iteration, we can only adapt the parameter $\theta_{i+1}$ of the model, and cannot directly apply the Bellman operator as in the tabular case. Moreover, we only have sampled transitions, rather the environment dynamics model $P$. It is desirable to choose a loss that is compatible with stochastic optimization, as an approximation for the Bellman operator. 

%In practical algorithms, the joint distribution model $\bm{Z}_i$ is approximated by the target network. We suppose for each iteration $i$, $\bm{Z}_{i}(s,a) := \bm{Z}(s,a,z;\theta_{i})$ where $\theta_{i}$ parameterizes the joint distribution model $\bm{Z}_{i}$ and $z \sim p(z)$ is noise parameter with distribution $p(z)$. Our objective is to find the optimal parameter $\theta_{i+1}$ to make the online network $\bm{Z}_{i+1}=\bm{Z}(s,a,z;\theta_{i+1})$ match the joint distribution $\mathcal{T}^\pi \bm{Z}_i$ in policy evaluation setting, and match joint distribution $\mathcal{T} \bm{Z}_i$ in policy optimization setting. In the following discussion, we focus on policy optimization setting, and analysis for policy evaluation setting is similar. 

We achieve this by minimizing the Maximum Mean Discrepancy (MMD) between joint distribution $\bm{\mu}_{i+1}$ and $\mathcal{T} \bm{\mu}_i$, which is defined as the equation below. 
\begin{equation}
\label{eq-mmd-definition}
    \text{MMD}^2(p, q; k) = \mathbb{E}_{x, x' \sim p}k(x, x') - 2\mathbb{E}_{x\sim p, y \sim q}k(x, y) + \mathbb{E}_{y, y' \sim q} k(y, y'),
\end{equation}
where $k(\cdot, \cdot)$ is some kernel function and MMD is defined upon $k$, and each pair of random variable $(x, x'), (x, y), (y, y')$ are independent. In our scenario, we use $\text{MMD}^2(\bm{\mu}_{i+1}(s,a), \mathcal{T} \bm{\mu}_i(s,a);k)$ as the temporal difference loss. 
The reason why we choose MMD as the objective function is that MMD is both a metric on distribution and easy to optimize with sampled transitions. 
%\textcolor{blue}{As we can see from the definition, MMD is easy to optimize with sampled transitions.}
%\textcolor{blue}{One may wonder if it is necessary to prove the contraction of Bellman operator under MMD, as in previous work on 1-dimentional distributional RL with MMD\cite{MMD-DQN}. However, we argue that, if the operator is proved to be contraction under one metric, then iterative applying the operator will converge. To ``apply" the operator, we just need a loss that is a metric, so that when the loss is zero we can guarantee that the two distribution is identical.} 
%The reason why we choose MMD as the objective function is that MMD is both a metric on distribution and easy to optimize. 
The original paper of MMD \citep{gretton2012kernel} proves that MMD is a metric on distribution when kernel $k$ is characteristic, from which we can prove that
\begin{equation} \label{eq-zero-mmd-apply-operator}
    \bm{\mu}_{i+1} = \mathcal{T} \bm{\mu}_i \iff \forall (s,a) \in \mathcal{S} \times \mathcal{A}, \text{MMD}^2(\bm{\mu}_{i+1}(s,a),\mathcal{T} \bm{\mu}_i(s,a);k) = 0,
\end{equation}
when the kernel $k$ is characteristic. If the MMD metric is optimized to zero and the appropriate kernel is selected, 
%we have the exact value adaptation of 
$\bm{\mu}_{i+1}$ is the exact result of applying the joint distributional Bellman operator. 
% We refer readers to Section 3.4 where we detail how we choose our kernel function. % $k(x, y) = \exp(-\|x - y\|_2^2 / h)$

In the algorithmic aspect, $\mathcal{T} \bm{\mu}_i(s,a)$ serves as the target distribution, $\bm{\mu}_{i+1}(s,a)$ serves as the prediction from online network, and we use $\text{MMD}^2(\bm{\mu}_{i+1}(s,a),\mathcal{T} \bm{\mu}_i(s,a);k)$ as temporal difference loss to match the online prediction and target distribution. Next, we establish the method to optimize $\text{MMD}^2(\bm{\mu}_{i+1}(s,a), \mathcal{T} \bm{\mu}_i(s,a);k)$ with transition samples. Note that we use $\bm{\mu}(s,a;\theta_i)$ to represent $\bm{\mu}_i(s,a)$, so the temporal difference loss can also be written as $\text{MMD}^2(\bm{\mu}(s,a;\theta_{i+1}), \mathcal{T} \bm{\mu}(s,a;\theta_{i});k)$. We use equation \eqref{eq-mmd-definition} to estimate the gradient of this squared MMD loss with respect to parameter $\theta_{i+1}$. Specifically, the first term in equation \eqref{eq-mmd-definition} can be unbiasedly estimated by drawing multiple independent samples from the online network $\bm{\mu}(s,a;\theta_{i+1})$; the second term of equation \eqref{eq-mmd-definition} can be unbiasedly estimated by drawing independent samples from the online network $\bm{\mu}(s,a;\theta_{i+1})$ and from the target distribution $\mathcal{T} \bm{\mu}(s,a;\theta_{i})$\footnote{We only require each sample from the online network $\bm{\mu}(s,a;\theta_{i+1})$ to be independent of every sample from the target distribution $\mathcal{T} \bm{\mu}(s,a;\theta_{i})$, and multiple samples from  the target distribution $\mathcal{T} \bm{\mu}(s,a;\theta_{i})$ can be dependent of each other.}. % From a transition sample $(s,a,\bm{r},s')$. 
%From transition sample $(s,a,\bm{r},s')$, we can prove that by computing the action $a'=\argmax_{a}(\mathbb{E}_{\sum})\bm{\mu}(s',a;\theta_{i})$ which is the action that maximizes expected return in state $s'$, $\gamma \bm{Z} + \bm{r}$ follows the distribution $\mathcal{T} \bm{\mu}(s,a;\theta_{i})$, where $\bm{Z}$ is a sample from $\bm{\mu}(s',a';\theta_i)$. 
Batch of samples from the target joint distribution $\mathcal{T} \bm{\mu}(s,a;\theta_{i})$ can be collected from only one transition sample $(s,a,\bm{r},s')$, and Lemma 6 in Appendix A.1 provides detailed proofs. For the third term in equation \eqref{eq-mmd-definition}, it has no gradient with respect to the parameter $\theta_{i+1}$, and we can safely ignore it during optimization. In summary, the gradient of the temporal difference loss $\text{MMD}^2$ can be estimated without bias by transition samples. Algorithm~\ref{algorithm-1} summarizes the above analysis and shows how our method computes the gradient estimates of the temporal difference loss $\text{MMD}^2$. 

% \textcolor{blue}{MMD is defined in terms of expectation. In practice, we calculate loss based on samples from distribution to get an unbiased estimation of MMD. Here, we use stochastic samples rather than deterministic samples as in MMDQN, to capture the rich information of joint return distributions. To be specific, we model the return distribution as $\bm{Z}(s,a,z;\theta_{i})$ where $\theta_{i}$ parameterizes the joint distribution $\bm{\mu}_{i}$ and $z \sim p(z)$ is noise parameter with distribution $p(z)$. By sampling the noise $z$, we can get stochastic samples $x = \bm{Z}(s,a,z;\theta_{i})$ from distribution. With stochastic samples, we can approximate the expected MMD loss then the number of samples approach infinity. Algorithm 1 give details on how to computes the gradient of the MMD metric based on sampled data. }

% \textcolor{red}{replace this paragraph by the analysis of unbiased estimation}

\iffalse
For the optimization of MMD metric, 
since the third term in equation \ref{eq-mmd-definition} has no gradient to $p$, we have the gradient form of MMD metric with respect to parameter $\theta_{i+1}$ as follows: 
\begin{align}
    &\ \ \ \ \nabla_{\theta_{i+1}}\text{MMD}^2(\bm{Z}_{i+1}(s,a), \mathcal{T} \bm{Z}_i(s,a); k) \nonumber \\
    &= \nabla_{\theta_{i+1}}\left[\mathbb{E}_{x, x' \sim \bm{Z}_{i+1}(s,a)}k(x, x') - 2\mathbb{E}_{x\sim \bm{Z}_{i+1}(s,a), y \sim \mathcal{T} \bm{Z}_i(s,a)}k(x, y)\right] \label{eq-gradient-mmd}
\end{align}

The benefits of using MMD is that, in the above gradient form both the first and the second expectation term can be unbiasedly estimated with batched data. We detail this claim in the next paragraph. 

Suppose we are given a transition sample $(s,a,r,s',a')$ where $a'$ maximize the expected total return same as equation \ref{eq-optimal-op-where}. We sample $x_{1:N} \stackrel{i.i.d.}{\sim} \bm{Z}_{i+1}(s,a)$ and $x_{1:N}^{target} \stackrel{i.i.d.}{\sim} \bm{Z}_i(s',a')$, and compute $y_{1:N}$ by $y_i= r + \gamma x_{i}^{target}$ for $i=1,2,\cdots,N$. It is clear that $k(x_i, x_j)$ forms the sample in the first term when $i \neq j$, since $x_i, x_j$ are independently sampled. Also, $y_{1:N}$ form the samples from distribution $\mathcal{T} \bm{Z}_i(s,a)$ and $k(x_i, y_j)$ forms the sample in the second term of equation \ref{eq-gradient-mmd} for all $(i,j)$. In summary, $x_{1:N}$ and $y_{1:N}$ can be used to give an unbiased gradient estimate for equation \ref{eq-gradient-mmd}.

% \blue{Compared to previous metric, show why MMD is easy to optimize}
Algorithm 1 wraps up discussions above and shows how HRDRL computes the gradient of the MMD metric based on sample data. 
\fi

\iffalse
\begin{algorithm}[]
\caption{Optimization of MMD metric by transition samples}\label{algorithm-1}
\begin{algorithmic}[1]
\STATEx \textbf{Require: } Number of samples $M$, kernel $k$, discount factor $\gamma \in (0, 1)$, policy $\pi$ if performing policy evaluation
\STATEx \textbf{Require: } Joint distribution network $\bm{\mu}(s,a;\theta)$
\STATEx \textbf{Input: } Transition sample $(s, a, \bm{r}, s')$
\STATEx \textbf{Input: } Online network parameter $\theta$, target network parameter $\theta'$
\STATEx \textbf{Output: } Gradient estimation of MMD with respect to $\theta$
\IF {Policy evalution setting}
    \STATE $a' \sim \pi(\cdot|s')$
\ELSE
    \STATE $a' \leftarrow \argmax_{a} \frac{1}{M}\sum_{m=1}^M \sum_{n=1}^N (\bm{Z}_{m})_n $, where $\bm{Z}_{1:M} \stackrel{i.i.d.}{\sim} \bm{\mu}(s', a;\theta')$. 
\ENDIF
\STATE Sample $\bm{Z}_{1:M} \stackrel{i.i.d.}{\sim} \bm{\mu}(s,a;\theta)$
\STATE Sample $\bm{Z}_{1:M}^{next} \stackrel{i.i.d.}{\sim} \bm{\mu}(s',a';\theta')$
\STATE $\bm{Z}_i^{target} \leftarrow \bm{r} + \gamma \bm{Z}_i^{next}$, for every $1 \leq i \leq M$
\STATE $\text{MMD}^2 \leftarrow \sum_{1 \leq i \leq M} \sum_{1 \leq j \leq M, j \neq i} \left[ k(\bm{Z}_i, \bm{Z}_j) - 2k(\bm{Z}_i, \bm{Z}_j^{target})  + k(\bm{Z}_i^{target}, \bm{Z}_j^{target})\right]$
\STATE \textbf{return} $\nabla_{\theta} \text{MMD}^2$

\end{algorithmic}
\end{algorithm}
\fi

\begin{algorithm}[]
\caption{Gradient estimation of $\text{MMD}^2$ loss by transition samples}\label{algorithm-1}
\begin{algorithmic}[1]
\STATEx \textbf{Require: } Number of samples $M$, kernel $k$, discount factor $\gamma \in (0, 1)$
\STATEx \textbf{Require: } Joint distribution network $\bm{\mu}(s,a;\theta)$
\STATEx \textbf{Input: } Transition sample $(s, a, \bm{r}, s')$
\STATEx \textbf{Input: } Online network parameter $\theta$, target network parameter $\theta'$
\STATEx \textbf{Output: } Gradient estimation of MMD with respect to $\theta$
    \STATE $a' \leftarrow \argmax_{a} \frac{1}{M}\sum_{m=1}^M \sum_{n=1}^N (\bm{Z}_{m})_n $, where $\bm{Z}_{1:M} \stackrel{i.i.d.}{\sim} \bm{\mu}(s', a;\theta')$. 
\STATE Sample $\bm{Z}_{1:M} \stackrel{i.i.d.}{\sim} \bm{\mu}(s,a;\theta)$ (samples from online network)
\STATE Sample $\bm{Z}_{1:M}^{next} \stackrel{i.i.d.}{\sim} \bm{\mu}(s',a';\theta')$ 
%\STATE $\bm{Z}_i^{target} \leftarrow \bm{r} + \gamma \bm{Z}_i^{next}$, for every $1 \leq i \leq M$
\STATE $\bm{Y_i} \leftarrow \bm{r} + \gamma \bm{Z}_i^{next}$, for every $1 \leq i \leq M$ (samples from target distribution)
%\STATE $\text{MMD}^2 \leftarrow \sum_{1 \leq i \leq M} \sum_{1 \leq j \leq M, j \neq i} \left[ k(\bm{Z}_i, \bm{Z}_j) - 2k(\bm{Z}_i, \bm{Z}_j^{target})  + k(\bm{Z}_i^{target}, \bm{Z}_j^{target})\right]$
\STATE $\text{MMD}^2 \leftarrow \sum_{1 \leq i \leq M} \sum_{1 \leq j \leq M, j \neq i} \left[ k(\bm{Z}_i, \bm{Z}_j) - 2k(\bm{Z}_i, \bm{Y}_j)  + k(\bm{Y}_i, \bm{Y}_j)\right]$
\STATE \textbf{return} $\nabla_{\theta} \text{MMD}^2$

\end{algorithmic}
\end{algorithm}

\subsection{Network Architecture and Implementation Details}

% We illustrate our network architecture in Figure \ref{img-network-architecture}. 
For a given state-action pair $(s,a)$, we use the value network of DQN~\citep{mnih2013playing} to compute the low-dimensional (512d) embedding of state $s$, and replace the final layer of DQN network to output a vector with $M \times N \times |\mathcal{A}|$ dimensions, representing $M$ samples from the joint return distribution from $N$ sources of reward for every action. % and outputs corresponding to action $a$ to get the embedding $c(s,a)$. We use gaussian distribution $N(0,1)$ as the noise distribution $p(z)$, and multple samples of random noise $z \sim p(z)$ is concatenated to embedding $c(s,a)$, then feed forward with MLP to output the samples of \textcolor{red}{$\bm{\mu}(s,a)$}. The output of neural network is $N$-dimensional vector, representing one sample of $N$ hybrid-source return.

We follow the kernel selection in MMDQN~\citep{nguyen2020distributional} and apply the Gaussian kernel function with mixed bandwidth\footnote{Gaussian kernel is proved to be characteristic~\citep{gretton2012kernel}, so the MMD distance with Gaussian kernel is a metric. It follows that when we use Gaussian kernels with mixed bandwidth, equation \eqref{eq-zero-mmd-apply-operator} still holds. }. % \textcolor{red}{characteristic kernel}
% \textcolor{red}{
%Here we make our second modification, to adapt to the different reward scale under hybrid reward setting. However, the reward scale could be different for different reward sources. By using the original L2 norm in gaussian kernel, we may ignore the changes for reward sources with small scales. To deal with such problem, we adopt a re-weighted L2 norm rather than original L2 norm in 1-dimensional setting, which can be expressed as follows: }
% \textcolor{red}{Change the norm to re-weighted norm here!!!}
\begin{align}
    k(x, x') &= \sum_{i=1}^{M} k_{w_i}(x,x'), \\
    \text{ where } k_{w_i}(x, x') &= e^{-\frac{\|x - x'\|_2^2}{w_i}}.
\end{align}

Each $w_i$ can be seen as the square of bandwidth in a Gaussian kernel. %It is worth noting that when the squared bandwidth $w_i > 0$ is too small or too large, the kernel function converges to 0 or 1 respectively and the gradients for MMD converge to zero. 
We choose the value of squared bandwidth $w_i$ with diverse ranges, to make sure that all scales of reward don't suffer from gradient vanishing. In Appendix A.3.4 and A.3.5, we test the performance of different network architectures and different bandwidth sets to find the optimal network architecture and bandwidth configurations. 

\iffalse
\textcolor{red}{We also keep an exponential moving average of expectation of each dimension in TD target, $r_n + \gamma \mathbb{E}[Z_{i,n}]$, and use those statistics to reweight L2 norm. 
This trick also enables us to deal with no-reward clipping setting in Atari Games. 
}

\fi

==> Distributional RL with Multiple Reward/src/5-method.tex <==
\section{Hybrid Reward Distributional Reinforcement Learning}

In this paper, we propose to capture the correlated randomness from multiple reward sources, forcing the agent to gain more knowledge about the environment and learn better representations. Specifically, we consider the joint distribution of returns from different reward sources. 
First, we introduce the joint distributional bellman operator and establish its convergence. We correct the misunderstanding in existing work~\citep{bellemare2017distributional,nguyen2020distributional}, that we must use the same metric for proving convergence and as training loss. We illustrate that, once the convergence of Bellman operator is proved under certain metric, we can use other metrics than the metric for proving convergence, as training loss to approximate the Bellman operator. 
Second, we introduce an empirical algorithm, which approximates Bellman operator through stochastic optimization with deep neural networks. Inspired by MMDQN~\citep{nguyen2020distributional}, we introduce a temporal difference loss based on Maximum Mean Discrepancy over joint return distributions.
Finally, we give full implementation details of our method, including network architectures and algorithms \sout{for loss computation}. % In order to adapt to multiple reward sources with different reward scale, we also introduce re-weighted norm with adaptive weight for gaussian kernels in the MMD loss to balance between rewards from different sources.

%\textcolor{blue}{In this paper, we consider the joint return distribution under the hybrid reward setting. First, we introduce the joint distributional bellman operator and establish its convergence. To approximate such operator through stochastic optimization in practical algorithm with deep neural networks, we then introduce a temporal difference loss based on Maximum Mean Discrepancy over joint return distributions, as inspired by \cite{}. Finally we give full implementation details of our method, including network architectures and loss computations. }

%\textcolor{red}{Both the theoretical and algorithmic parts of our method can be seen as extensions of existing theoretical and algorithmic works on 1-dimension to K-dimension. It is worth mentioning that such extension is non-trivial, in that we fix some issues and make some adaptations to K-dimension. We find the 1-dimensional contraction proof in \cite{C51} skip some steps, making it hard to follow, therefore we give a more detailed contraction proof under the joint distribution setting. While the original algorithm in 1-dimension takes use of deterministic samples from return distribution, we propose to estimate stochastic samples with more flexibility to approximate the whole return distribution as the number of samples approach infinite. In order to deal with different scale of reward from hybrid sources, we also introduce re-weighted norm for gaussian kernels in the MMD loss. }


%We first define the hybird-source return as a K-dimensional random variable, and introduce Wasserstein metric $Wp$ the joint distribution and  on the settings and establish the convergence of the joint distributional bellman operator. 


%In this section, we firstly focus on the settings and convergence analysis for learning the joint value distribution of hybrid-source return. We prove that iteratively \textcolor{blue}{applying} %adapting by 
%joint distributional Bellman operator will make the estimation converge to the ground truth value distribution. 
%We then introduce a temporal difference error based on metric over joint value distribution, and explain why optimizing the loss can be approximated as applying joint distributional Bellman operator. 
%Finally we give full implementation details of our method, including network architectures and loss computations. 


\subsection{Definitions and Settings}

%We define $\vec{Z}^\pi(s,a)$ as
We consider the joint return distribution $\bm{Z}^\pi(s,a)$ under policy $\pi$ as
\begin{align}
    \bm{Z}^\pi(s,a) &\stackrel{D}{\coloneqq} \sum_{t=0}^\infty \gamma^t \bm{r}_t, \\
    \text{ where } s_0 &= s, a_0 = a, \bm{r}_t \sim R(\cdot|s_t, a_t), s_{t+1} \sim P(\cdot|s_t, a_t), a_{t+1} \sim \pi(\cdot|s_{t+1}).
\end{align}

%We can interpret $\vec{Z}^\pi(s,a)$ as the joint distribution for the discounted return of multiple source reward. 
The $i$-th dimension of $\bm{Z}^\pi(s,a)$ is the random variable for the $i$-th source of discounted return, and different dimensions in $\bm{Z}^\pi(s,a)$ can be correlated. We use $\bm{Z}: \mathcal{S} \times \mathcal{A} \rightarrow \mathcal{P}(\mathbb{R}^K)$ to denote a joint return distribution model, where $\bm{Z}(s,a) \in \mathcal{P}(\mathbb{R}^K)$ is the joint distribution predicted by the model on state action pair $(s,a)$ of future returns over multiple reward sources. The goal of our algorithm is to let model $\bm{Z}$ to be as close to $\bm{Z}^\pi$ as possible in policy evaluation setting, i.e. to model the real joint return distribution. 

To measure how close two $K$-dimensional joint distributions are, we adopt Wasserstein metric $W_p$.  %If we have 
For two joint distributions $\mu, \nu \in \mathcal{P}(\mathbb{R}^K)$, the p-Wasserstein metric $W_p(\mu, \nu)$ on Euclidean distance $d$ is given by: 
\begin{equation}
    W_p(\mu, \nu) = \left(\inf_{f \in \Gamma(\mu, \nu)} \int_{\mathbb{R}^K \times \mathbb{R}^K} d(x, y)^p f(x,y) d^K x d^K y \right)^{1/p}
    %W_p(\mu, \nu) = \left(\inf_{f \in \Gamma(\mu, \nu)} \int_{\mathbb{R}^K \times \mathbb{R}^K} d(x, y)^p  \mathrm{d} f(x,y) \right)^{1/p}
\end{equation}
where $\Gamma(\mu, \nu)$ is the collection of all distributions with marginal distribution $\mu$ and $\nu$ on the first and second $K$ random variables %factors 
respectively. The Wasserstein distance can be interpreted as the minimum moving distance to move all the mass from distribution $\mu$ to distribution $\nu$. 

To measure the distance between two joint distribution models $\bm{Z}_1$ and $\bm{Z}_2$, %$W_1$ and $W_2$, 
we take the maximum Wasserstein distance over all state action pairs, formalized in the equation below. 
\begin{equation}
    %d_p(W_1, W_2) := \max_{s,a} W_p(W_1(s,a), W_2(s,a)). 
\bar{d}_p(\bm{Z}_1, \bm{Z}_2) := \max_{s,a} W_p(\bm{Z}_1(s,a), \bm{Z}_2(s,a)) 
\end{equation}
We will use $\bar{d}_p$ to establish the convergence of the joint distributional Bellman operator. 
\iffalse
\begin{lemma}
    $\bar{d}_p$ is a metric over joint return distributions.
\end{lemma}
\fi

\subsection{Convergence of Joint Distributional Bellman Operator}
%\textcolor{blue}{We extend the theoretical results on distributional bellman operator from 1-dimension distribution in C51, to high-dimensional distribution in our case. It is worth mentioning that it is non-trivial to extend the theoretical results to high-dimensional distribution, where the wasserstein distance does not have nice formulation as in 1-dimensional case. Detailed proofs can be found in Appendix.  }
%The theory framework is mainly based on C51 paper \citep{bellemare2017distributional}, but our conclusion is the extension of theirs and require more work than C51. 
We define the joint distributional Bellman evaluation operator $\mathcal{T}^\pi$ as
\begin{align}
    \mathcal{T}^\pi \bm{Z}(s_t,a_t) &\stackrel{D}{\coloneqq} \bm{r}_t + \gamma \bm{Z}(s_{t+1}, a_{t+1}) \\
    \text{ where } & \bm{r}_t \sim R(\cdot|s_t,a_t), s_{t+1} \sim P(\cdot|s_t,a_t), a_{t+1} \sim \pi(\cdot|s_{t+1})
\end{align}

The below theorem shows that $\mathcal{T}^\pi$ is a $\gamma$-contraction operator on $\bar{d}_p$. % We provide detailed proof of Theorem 1 in Appendix A. 

\begin{theorem}
    For two joint distribution models $\bm{Z}_1$ and $\bm{Z}_2$, %$W_1$ and $W_2$, 
    we have
    \begin{equation}
        %d_p(\mathcal{T}^\pi W_1, \mathcal{T}^\pi W_2) \leq \gamma d_p(W_1, W_2)
        \bar{d}_p(\mathcal{T}^\pi \bm{Z}_1, \mathcal{T}^\pi \bm{Z}_2) \leq \gamma \bar{d}_p(\bm{Z}_1, \bm{Z}_2).
    \end{equation}
\end{theorem}
We consider the following scenario: initially we have a joint distribution model $\bm{Z}_0: \mathcal{S} \times \mathcal{A} \rightarrow \mathcal{P}(\mathbb{R}^K)$, and iteratively adapt the model by $\bm{Z}_{i+1} = \mathcal{T}^\pi \bm{Z}_i $. 
According to Banach's fixed point theorem, operator $\mathcal{T}^\pi$ has a unique fixed point, which is $\bm{Z}^\pi$ by definition. 
%Since $\bm{Z}^\pi$ is the fix point of operator $\mathcal{T}^\pi$, 
The distance between $\bm{Z}_i$ and $\bm{Z}^\pi$ decays as $i$ increases. We have the following proposition: 
\begin{proposition}
    If $\bm{Z}_{i+1} = \mathcal{T}^\pi \bm{Z}_i $, then as $i \rightarrow \infty$, $\bm{Z}_i \rightarrow \bm{Z}^\pi$. 
\end{proposition}

We also provide contraction proof on expectation of the optimality operator.
%%%%%% \blue{Please check here}
The joint distributional Bellman optimality operator $\mathcal{T}$ is defined as
\begin{align}
    \mathcal{T}\bm{Z}(s_t,a_t) &\stackrel{D}{\coloneqq} \bm{r}_t + \gamma \bm{Z}(s_{t+1}, a') \label{eq-optimal-op} \\
    \text{ where } & \bm{r} \sim R(\cdot|s_t,a_t), s_{t+1} \sim P(\cdot|s_t,a_t), a'=\argmax_{a'} \mathbb{E} \sum_{k=1}^K Z_k(s_{t+1}, a') \label{eq-optimal-op-where}
\end{align}

\textcolor{red}{definition for E operator}

\begin{theorem}
    For two joint distribution models $\bm{Z}_1$ and $\bm{Z}_2$, %$W_1$ and $W_2$, 
    we have
    \begin{equation}
        %\vert \vert \mathbb{E} \mathcal{T} W_1 - \mathbb{E} \mathcal{T} W_2 \vert \vert_{\infty} \leq \gamma \vert \vert \mathbb{E}  W_1 - \mathbb{E} W_2 \vert \vert
        \vert \vert \mathbb{E} \sum_{k} (\mathcal{T} \bm{Z}_1)_k - \mathbb{E} \sum_{k} (\mathcal{T} \bm{Z}_2)_k \vert \vert_{\infty} \leq \gamma \vert \vert \mathbb{E}  \sum_{k}Z_{1,k} - \mathbb{E} \sum_{k}Z_{2,k} \vert \vert
    \end{equation}
\end{theorem}
%\textcolor{red}{redefine the expectation here! Should be sum over all sub-returns. }
where $Z_{\cdot,k}$ represents the marginal distribution for the $k$-th source-specific return.
%%%%%%

\begin{proposition}
    If $\bm{Z}_{i+1} = \mathcal{T} \bm{Z}_i $, then as $i \rightarrow \infty$, $\mathbb{E}[\sum_{k=1}^{K} Z_{i,k}] \rightarrow Q^*$%\mathbb{E}[\sum_{k=1}^{K} Z^{*}_{i,k}]$. 
\end{proposition}

The proposition 2 can be interpreted as following: as we iteratively apply the joint distributional Bellman optimality operator, the expected total return of the joint distribution predicted by the model $Z_i$ will converge to optimal value function. We refer the readers to the appendix for details proofs for all the lemmas, theorems, and propositions.


%There is a common misunderstanding in existing work that it is necessary to use the same metric to prove convergence and as training loss~\citep{bellemare2017distributional, nguyen2020distributional}. However, we argue that, convergence is the property of the operator itself, regardless of the metric. If the operator is proved to be contraction under one metric, then applying the operator iteratively will lead to convergence to a fixed point. In contrast, training loss is used to "apply" the operator. In fact, we can use any loss, as long as we can guarantee the distribution and its Bellman target are identical when the loss is minimized. 
%For example, in C51~\citep{bellemare2017distributional}, the Cramer distance is used implicitly in the projection step, and the projected operator is proved to be contraction under cramer distance. Then, we can apply this projected operator with KL-divergence, since KL-divengence is minimized if and only if two distributions are identical. \textcolor{red}{maybe we need to week the claim}
\textcolor{blue}{There is a common misunderstanding in existing works that we must use the same metric to prove convergence and as training loss~\citep{bellemare2017distributional, nguyen2020distributional}. We clarify that the metric for proving convergence and the metric for training loss play different roles, and are not necessarily the same metric. 
For example, Cramer distance is used to prove the contraction property of the projected Bellman operator in C51~\citep{pmlr-v84-rowland18a}. The contraction property leads to the convergence property. KL-divergence is used to approximate the projected operator in C51~\citep{bellemare2017distributional}. With infinite sampled transitions and expressive value networks, we can approximate the projected operator exactly when the KL-divergence is minimized. }


\subsection{Optimizing MMD as approximation for Bellman Operater}

%\textcolor{blue}{1. We extend existing distribution RL algorithm to high-dimensional? or we approximate the joint distributional bellman operator with xxx loss? 2. C51 is not easy to scale to high-dimensional. Sample-based method is much better.3. approximate continuous distribution with samples. logic is not clear yet. Try to figure out a good logic tomorrow. }

In practical algorithms, the joint distributional model $\bm{Z}_i$ is represented by deep neural network $\bm{Z}(s,a;\theta_{i})$ with parameter $\theta_i$. We cannot directly apply the Bellman operator as in tabular case. Moreover, we only have sampled transitions, rather the the environment dynamics model $P$. It is desirable to choose a loss that is compatible with stochastic optimization, as an approximation for Bellman operator. 

%In practical algorithms, the joint distribution model $\bm{Z}_i$ is approximated by the target network. We suppose for each iteration $i$, $\bm{Z}_{i}(s,a) := \bm{Z}(s,a,z;\theta_{i})$ where $\theta_{i}$ parameterizes the joint distribution model $\bm{Z}_{i}$ and $z \sim p(z)$ is noise parameter with distribution $p(z)$. Our objective is to find the optimal parameter $\theta_{i+1}$ to make the online network $\bm{Z}_{i+1}=\bm{Z}(s,a,z;\theta_{i+1})$ match the joint distribution $\mathcal{T}^\pi \bm{Z}_i$ in policy evaluation setting, and match joint distribution $\mathcal{T} \bm{Z}_i$ in policy optimization setting. In the following discussion, we focus on policy optimization setting, and analysis for policy evaluation setting is similar. 

We achieve this by minimizing the Maximum Mean Discrepancy (MMD) between joint distribution $\bm{Z}_{i+1}$ and $\mathcal{T} \bm{Z}_i$, which is defined as the equation below. 
\begin{equation}
\label{eq-mmd-definition}
    \text{MMD}^2(p, q; k) = \mathbb{E}_{x, x' \sim p}k(x, x') - 2\mathbb{E}_{x\sim p, y \sim q}k(x, y) + \mathbb{E}_{y, y' \sim q} k(y, y'),
\end{equation}
where $k(\cdot, \cdot)$ is some kernel function and MMD is defined upon $k$, and each pair of random variable in $(x, x'), (x, y), (y, y')$ are independent. In our scenario, we use $\text{MMD}^2(\bm{Z}_{i+1}, \mathcal{T} \bm{Z}_i)$ as the temporal difference loss. 
\textcolor{blue}{The reason why we choose MMD as the objective function is that MMD is both a metric on distribution and} \textcolor{red}{can be optimized with sampled transitions}. 
%\textcolor{blue}{As we can see from the definition, MMD is easy to optimize with sampled transitions.}
%\textcolor{blue}{One may wonder if it is necessary to prove the contraction of Bellman operator under MMD, as in previous work on 1-dimentional distributional RL with MMD\cite{MMD-DQN}. However, we argue that, if the operator is proved to be contraction under one metric, then iterative applying the operator will converge. To ``apply" the operator, we just need a loss that is a metric, so that when the loss is zero we can guarantee that the two distribution is identical.} 
%The reason why we choose MMD as the objective function is that MMD is both a metric on distribution and easy to optimize. 
The original paper of MMD \citep{gretton2012kernel} proves that MMD is a metric on distribution when kernel $k$ is characteristic, from which we can prove that
\begin{equation}
    \bm{Z}_{i+1} = \mathcal{T} \bm{Z}_i \iff \forall (s,a) \in \mathcal{S} \times \mathcal{A}, \text{MMD}^2(\bm{Z}_{i+1}(s,a),\mathcal{T} \bm{Z}_i(s,a);k) = 0,
\end{equation}
when the kernel $k$ is characteristic. If the MMD metric is optimized to zero and appropriate kernel is selected, 
%we have the exact value adaptation of 
$Z_{i+1}$ is the result of exactly applying the joint distributional Bellman operator. 
We refer reader to Section 3.4 where we detail how we choose of our kernel function. % $k(x, y) = \exp(-\|x - y\|_2^2 / h)$

\textcolor{blue}{MMD is defined in terms of expectation. In practice, we calculate loss based on samples from distribution to get an unbiased estimation of MMD. Here, we use stochastic samples rather than deterministic samples as in MMDQN, to capture the rich information of joint return distributions. To be specific, we model the return distribution as $\bm{Z}(s,a,z;\theta_{i})$ where $\theta_{i}$ parameterizes the joint distribution model $\bm{Z}_{i}$ and $z \sim p(z)$ is noise parameter with distribution $p(z)$. By sampling the noise $z$, we can get stochastic samples $x = \bm{Z}(s,a,z;\theta_{i})$ from distribution $\bm{Z}_i$. With stochastic samples, we can approximate the expected MMD loss then the number of samples approach infinity. Algorithm 1 give details on how to computes the gradient of the MMD metric based on sampled data. 
}

\textcolor{red}{replace this paragraph by the analysis of unbiased estimation}

\iffalse
For the optimization of MMD metric, 
since the third term in equation \ref{eq-mmd-definition} has no gradient to $p$, we have the gradient form of MMD metric with respect to parameter $\theta_{i+1}$ as follows: 
\begin{align}
    &\ \ \ \ \nabla_{\theta_{i+1}}\text{MMD}^2(\bm{Z}_{i+1}(s,a), \mathcal{T} \bm{Z}_i(s,a); k) \nonumber \\
    &= \nabla_{\theta_{i+1}}\left[\mathbb{E}_{x, x' \sim \bm{Z}_{i+1}(s,a)}k(x, x') - 2\mathbb{E}_{x\sim \bm{Z}_{i+1}(s,a), y \sim \mathcal{T} \bm{Z}_i(s,a)}k(x, y)\right] \label{eq-gradient-mmd}
\end{align}

The benefits of using MMD is that, in the above gradient form both the first and the second expectation term can be unbiasedly estimated with batched data. We detail this claim in the next paragraph. 

Suppose we are given a transition sample $(s,a,r,s',a')$ where $a'$ maximize the expected total return same as equation \ref{eq-optimal-op-where}. We sample $x_{1:N} \stackrel{i.i.d.}{\sim} \bm{Z}_{i+1}(s,a)$ and $x_{1:N}^{target} \stackrel{i.i.d.}{\sim} \bm{Z}_i(s',a')$, and compute $y_{1:N}$ by $y_i= r + \gamma x_{i}^{target}$ for $i=1,2,\cdots,N$. It is clear that $k(x_i, x_j)$ forms the sample in the first term when $i \neq j$, since $x_i, x_j$ are independently sampled. Also, $y_{1:N}$ form the samples from distribution $\mathcal{T} \bm{Z}_i(s,a)$ and $k(x_i, y_j)$ forms the sample in the second term of equation \ref{eq-gradient-mmd} for all $(i,j)$. In summary, $x_{1:N}$ and $y_{1:N}$ can be used to give an unbiased gradient estimate for equation \ref{eq-gradient-mmd}.

% \blue{Compared to previous metric, show why MMD is easy to optimize}
Algorithm 1 wraps up discussions above and shows how HRDRL computes the gradient of the MMD metric based on sample data. 
\fi

\begin{algorithm}[]
\caption{Optimization of MMD metric by transition samples}\label{algorithm-1}
\begin{algorithmic}[1]
\STATEx \textbf{Require: } Number of samples $N$, kernel $k$, discount factor $\gamma \in (0, 1)$, policy $\pi$ if performing policy evaluation
\STATEx \textbf{Require: } Joint distribution network $\bm{Z}(s,a,z;\theta)$
\STATEx \textbf{Input: } Transition sample $(s, a, r, s')$
\STATEx \textbf{Input: } Online network parameter $\theta$, target network parameter $\theta'$
\STATEx \textbf{Output: } Gradient estimation of MMD with respect to $\theta$
\IF {Policy evalution setting}
    \STATE $a' \sim \pi(\cdot|s')$
\ELSE
    \STATE $a' \leftarrow \argmax_{a'} \sum_{k=1}^K\frac{1}{N}\sum_{i=1}^N \bm{Z}(s', a',z_i;\theta')_k $, where $z_{1:N} \sim p(z)$. 
\ENDIF
\STATE $x_i \leftarrow \bm{Z}(s,a,z_i;\theta)$, where $z_i \sim p(z)$, for every $1 \leq i \leq N$
\STATE $x_i^{target} \leftarrow \bm{Z}(s,a,z_i^{target};\theta')$, where $z_i^{target} \sim p(z)$, for every $1 \leq i \leq N$
\STATE $y_i \leftarrow r + \gamma x_i^{target}$, for every $1 \leq i \leq N$
\STATE $\text{MMD}^2 \leftarrow \sum_{1 \leq i \leq N} \sum_{1 \leq j \leq N, j \neq i} \left[ k(x_i, x_j) - 2k(x_i, y_j)  + k(y_i, y_j)\right]$
\STATE \textbf{return} $\nabla_{\theta} \text{MMD}^2$

\end{algorithmic}
\end{algorithm}

\subsection{Network Architecture and Implementation Details}

We illustrate our network architecture in Figure \ref{img-network-architecture}. For a given state-action pair $(s,a)$, we use the Nature DQN network to compute the embedding of state $s$ with all possible actions, and select the embedding corresponding to action $a$ to get the embedding $c(s,a)$. We use gaussian distribution $N(0,1)$ as the noise distribution $p(z)$, and multple samples of random noise $z \sim p(z)$ is concatenated to embedding $c(s,a)$, then feed forward with MLP to output the samples of $\bm{Z}(s,a)$. The output of neural network is $K$-dimensional vector, representing one sample of $K$ hybrid-source return.

\textcolor{red}{replace network architecture part, and graph}
\iffalse
\begin{figure}
  \centering
  \includegraphics[width=12cm]{files/hrmmd.pdf}
  \caption{Network architecture for joint distribution model. }
  \label{img-network-architecture}
\end{figure}
\fi

We follow the kernel selection in MMDQN \citep{nguyen2020distributional} and apply the gaussian kernel function with mixed bandwidth. \textcolor{red}{characteristic kernel}

% \textcolor{red}{
%Here we make our second modification, to adapt to the different reward scale under hybrid reward setting. However, the reward scale could be different for different reward sources. By using the original L2 norm in gaussian kernel, we may ignore the changes for reward sources with small scales. To deal with such problem, we adopt a re-weighted L2 norm rather than original L2 norm in 1-dimensional setting, which can be expressed as follows: }
% \textcolor{red}{Change the norm to re-weighted norm here!!!}

\begin{align}
    k(x, x') &= \sum_{i=1}^{B} k_{b_i}(x,x') \\
    \text{ where } k_b(x, x') &= e^{-\frac{\|x - x'\|_2^2}{b}}
\end{align}

It is worth noting that when the bandwidth $b_i > 0$ is too small or too large, the kernel function converge to 0 or 1 respectively and the gradient for MMD converge to zero. We choose the value of bandwidth $b_i$ with diverse range, specifically $b_i = 2^{i-2}$ for each $1 \leq i \leq 8$, to make sure that all scales of reward don't suffer from gradient vanishing. 

\iffalse
\textcolor{red}{We also keep an exponential moving average of expectation of each dimension in TD target, $r_k + \gamma \mathbb{E}[Z_{i,k}]$, and use those statistics to reweight L2 norm. 
This trick also enables us to deal with no-reward clipping setting in Atari Games. 
}

\fi

==> Distributional RL with Multiple Reward/src/6-experiment.tex <==
\section{Experimental Results}

In our experiments\footnote{Our code for the experiments is available in the supplementary material.}, we provide empirical results to answer the following questions: 
\begin{itemize}
    \item On policy evaluation settings, can MD3QN accurately model the joint distribution of multiple sources of reward? 
    \item On policy optimization settings, can MD3QN learn a better policy compared to HRA and distributional RL algorithm on environments with multiple sources of reward? 
\end{itemize}

To answer the first question, we design a maze environment with a rich way to generate correlated sources of rewards, and compare the joint distribution predicted by our method with the true joint distribution $\bm{\mu}^\pi$. The detailed setting of the environment and results is shown in Section 5.1. 

To answer the second question, we use several Atari games with multiple sources of reward, and provide training curve results of MD3QN compared to previous work HRA which deals with multiple sources of reward. The detailed setting of the environment and results is shown in Section 5.2. 

\subsection{Modeling Joint Return Distribution for Multi-Dimensional Reward Functions}

\iffalse
\begin{figure}[H]
  \centering
  \begin{subfigure}[b]{0.45\linewidth}
      \centering
      \includegraphics[width=4.0cm]{files/exp2-case-study.png}
      \caption{}
      \label{3-loss-1}
  \end{subfigure}
%   \hfill
  \begin{subfigure}[b]{0.45\linewidth}
      \centering
      \includegraphics[width=4.0cm]{files/exp2-case-study.png}
      \caption{}
      \label{3-cosine}
  \end{subfigure}
  \caption{ (placeholder) Case study for joint distribution modeling on Atari games. }
\end{figure}
\fi

In this experiment, we validate the capacity of MD3QN to model the joint return distribution for multiple sources of rewards on the policy evaluation setting with pixel inputs. The experiment is performed on the maze environments with rich reward correlation signals described as follows. 

% The triangle represents the agent, and different sources of reward are represented by squares with different colors. The agent cannot pass walls in black, and colored wall can only be passed in one way, where yellow walls can be passed from the top or from the left, and red walls can be passed from the bottom or from the right.

Figure \ref{fig-maze-env} illustrates three maze environments with different reward correlation properties. % In all of these environments, each block may have paths to adjacent blocks, with some paths blocked by walls, and some of the blocks contain a specific source of reward. 
The agent (represented by the triangle) is initially located at a specific position in the maze, and the policy $\pi$ is a fixed policy to uniformly choose one direction at random and try to move. If the agent is blocked by the walls in that direction\footnote{Colored walls can only be passed in one way, where yellow walls can be passed from the top or from the left, and red walls can be passed from the bottom or from the right.}, or the agent is trying to return to a previous position, the move has no effect, otherwise, the agent moves in that direction for one block.  Each color of the square in the maze represents one source of reward. When the agent reaches the position with reward, it receives a reward of the source aligned with the color of the square\footnote{More detailed description of how reward is set in these three environments is provided in Appendix A.2.}. The rules described above are general enough to enable the design of diversely correlated sources of rewards detailed below. 

Figure \ref{fig-maze-env-1} shows a maze environment with two exclusive sources of rewards. Once the agent obtains a reward from one side, it cannot obtain the reward from the other side.  Figure \ref{fig-maze-env-2} shows a maze environment with two positively correlated sources of rewards, where the agent either gets no reward or gets both of the red and green rewards. Figure \ref{fig-maze-env-3} shows a maze environment with four correlated sources of rewards. In these three environments, the agent needs to capture the negative correlation, positive correlation, and the complex correlation in multi-dimensional rewards respectively to precisely model the joint return distribution.

% Moreover, the environment makes the blocks that agent has passed invalid and the agent cannot return to the previous block that have been entered. In the maze setting displayed in Figure 2, some pairs of reward source (e.g. red and green) will be exclusive of each other, while some pairs of reward source (e.g. blue and orange) will have strong dependency to each other.  

On each of the three mazes, we train the MD3QN agent for 5 iterations (1.25M frames) to model the joint distribution of all sources of reward, and compare the prediction of joint distribution by the model to the samples from the true distribution $\bm{\mu}^\pi$ on the initial state of the maze. The results are shown in Figure \ref{fig-result-maze}, where each point in the figure is a sample representing one possibility of future discounted return in each source of reward. The result shows that MD3QN accurately models the joint return distribution from different sources of reward. 

In Appendix A.3.1, we visualize the modeled joint distribution throughout the training process, where the joint distribution modeled by MD3QN gradually match the true distribution. 

It is also worth noting that the observation for the agent is based on pixels, computed by downsampling the image in Figure \ref{fig-maze-env} to the size of $84\times 84$, which requires the agent to extract information on high-dimensional inputs.
% On a collections of state-action pairs, we compare the joint distribution modeling by MD3QN and the ground truth joint value distribution. The ground truth distribution is obtained by rolling out trajectories $N=1000$ times and compute the discounted sum of each reward source in each trajectory. Figure 3(a) shows the mean MMD metric across all state collections between MD3QN's model and ground truth distribution, where x-axis is the training iterations. Figure 3(c) shows one case study for comparing modeled distribution by MD3QN and ground truth distribution with state shown in Figure 3(b).

\begin{figure}[]
  \centering
  \begin{subfigure}[b]{0.32\linewidth}
     \centering
     \includegraphics[trim={2cm 0 2cm 0},clip,width=3.5cm]{files/maze-exclusive.png}
     \caption{}
     \label{fig-maze-env-1}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.32\linewidth}
     \centering
     \includegraphics[trim={2cm 0 2cm 0},clip,width=3.5cm]{files/maze-inclusive.png}
     \caption{}
     \label{fig-maze-env-2}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.32\linewidth}
     \centering
     \includegraphics[trim={2cm 0 2cm 0},clip,width=3.5cm]{files/maze-multireward.png}
     \caption{}
     \label{fig-maze-env-3}
  \end{subfigure}
  \caption{Observation of initial states in maze environments. (a): maze environment ``maze-exclusive'' with two exclusive sources of rewards. (b): maze environment ``maze-identical'' with two positively correlated sources of rewards. (c): maze environment ``maze-multireward'' with four correlated sources of rewards. }
  \label{fig-maze-env}
\end{figure}

\begin{figure}[]
  \centering
  \includegraphics[width=\textwidth]{files/maze-exp/Maze.pdf}
%   \begin{subfigure}[b]{0.24\linewidth}
%       \centering
%       % \raisebox{3mm}{}
%       \includegraphics[trim={0.4cm 0 0.4cm 0},clip,width=3.4cm]{files/maze-exp/v1.png}
%       \caption{}
%       \label{101-state}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}[b]{0.24\linewidth}
%       \centering
%       \includegraphics[trim={0.4cm 0 0.4cm 0},clip,width=3.4cm]{files/maze-exp/v2.png}
%       \caption{}
%       \label{2-overall}
%   \end{subfigure}
%   \begin{subfigure}[b]{0.24\linewidth}
%       \centering
%       \includegraphics[trim={0.4cm 0 0.4cm 0},clip,width=3.4cm]{files/maze-exp/v0-d0d1.png}
%       \caption{}
%       \label{}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}[b]{0.24\linewidth}
%       \centering
%       \includegraphics[trim={0.4cm 0 0.4cm 0},clip,width=3.4cm]{files/maze-exp/v0-d2d3.png}
%       \caption{}
%       \label{}
%   \end{subfigure}
  % \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \caption{ Comparison between samples from joint distribution by MD3QN and samples from the true distribution $\bm{\mu}^\pi$ in three maze environments. The number of samples is set to be 200. (a): the result of ``maze-exclusive'' environment. (b): the result of ``maze-identical'' environment. (c): the result of ``maze-multireward'' environment of orange and blue reward sources. (d): the result of ``maze-multireward'' environment of green and red reward sources.}
  \label{fig-result-maze}
\end{figure}


\subsection{Performance on Atari Games} \label{section-exp-atari}

In this experiment, we compare MD3QN algorithm with Hybrid Reward Architecture~(HRA)~\citep{van2017hybrid} and MMDQN~\citep{nguyen2020distributional} on Atari games from Arcade Learning Environment \citep{bellemare2013arcade}. Our implementation of MD3QN is built upon the Dopamine framework \citep{castro18dopamine}. The hyper-parameter settings used by MD3QN and the environment settings are detailed in Appendix A.2.

We use six Atari games with multiple sources of rewards: AirRaid, Asteroids, Gopher, MsPacman, UpNDown, and Pong. In all of these six games, the primitive rewards can be decomposed into multiple sources of rewards as follows: 
\begin{itemize}
    \item In AirRaid and Asteroids, the agent gets different value of reward for killing different types of monsters. 
    \item In Gopher, the agent gets +80 reward for killing a monster and gets +20 reward for removing holes on the ground.
    \item In MsPacman, the agent gets \{+200, +400, +800, +1600\} reward for killing a monster and gets +10 reward for eating beans.
    \item In UpNDown, the agent gets +400 reward for killing an enemy car, +100 reward for reaching a flag, and +10 reward for being alive. 
    \item In Pong, the agent gets +1 reward for winning a round, and gets -1 reward for losing a round.
\end{itemize}

We decompose the primitive rewards into multi-dimensional rewards according to the above reward structure, and meanwhile keeping the total reward not changed. The details for the reward decomposition method is provided in Appendix A.2. The training curves of MD3QN compared to HRA~\citep{van2017hybrid} and MMDQN~\citep{nguyen2020distributional} are shown in Figure~\ref{fig-atari-curve}. 

\begin{figure}
  \centering
  \includegraphics[width=0.75\textwidth]{files/rebuttal/Atari_HRA_MMDQN.pdf}
  \caption{ Performance of MD3QN on Atari games compared to HRA and MMDQN. The shaded areas show the standard deviation across 3 seeds. }
  \label{fig-atari-curve}
\end{figure}

Figure \ref{fig-atari-curve} shows that MD3QN does not outperform MMDQN in performance under several Atari games. We suspect the reason why MD3QN cannot outperform MMDQN is that the performance of Atari games might not be related to the joint distribution. We look forward to further studies on how the additional information captured in distributional RL algorithms helps to improve the final performance, to better interpret the experimental results. Despite that, with the distributional information, MD3QN outperforms or matches the performance of HRA under all six games.

On Atari games, we also show the joint distributions modeled by MD3QN, which is detailed in Appendix A.3.2. Overall, both the reward correlation and the reward scale in the return distribution are reasonably captured by MD3QN. The joint distribution captured by MD3QN show different and reasonable reward correlation across different Atari games. 

To show the necessity of modeling the joint distribution, we add another experiment in Appendix A.3.3 showing that only modeling marginal distributions may fail in environments with multiple correlated constraints, from theory and experiment results. 

\iffalse
\subsection{Downstream task for MD3QN: RL with multiple constraints}

\begin{figure}
  \centering
  \hspace*{\fill}%
  \begin{subfigure}[b]{0.4\linewidth}
     \centering
     \includegraphics[height=3cm]{files/rebuttal/constraint_maze_small.png}
     \caption{}
     \label{fig-constraint-env}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.4\linewidth}
     \centering
     \includegraphics[height=3cm]{files/rebuttal/multiple_constraint.png}
     \caption{}
     \label{fig-constraint-result}
  \end{subfigure}
  \hspace*{\fill}%
  \caption{ (a): maze environment with multiple constraints: $Z^{\text{red}} \geq 0.8, Z^{\text{green}} \geq 0.8, Z^{\text{blue}} \geq 0.8$.  (b): probability of the agent to satisfy all constraints during evalution throughout the training process. }
  \label{fig-maze-env}
\end{figure}
\fi

\section{Conclusions}

In this work, we have proposed Multi-Dimensional Distributional DQN~(MD3QN), a distributional RL method that learns a multi-dimensional joint return distribution for multiple sources of rewards. The effectiveness of our method is verified on pixel-input environments in terms of both the quality of modeled joint distribution, and the final performance of learnt policies. % Building a reliable framework to learn a multi-dimensional joint distribution model in RL has significant importance for a highly informative model of the environment. 

In the future, it is possible to extend our framework to model the correlated randomness in achieving different goals with goal-conditioned RL, and in visiting different states with successor representation. We will leverage such informative modeling of the environment in terms of goals and successor states to develop novel RL algorithms in our future work.
%This is our first step towards capturing the correlation between different sources of randomness. It is possible to extend our method to capture the correlation between achieving different goals in hindsight methods, and the correlation between visiting different states in successor representation. Such information could be quite useful for the agent to understand the environment, and it is possible to derive even more powerful RL algorithms based on such joint distribution model. For example, if we know two goal states are correlated, we have to achieve the first goal before the second goal. Then we can ask our agent to focus on the first goal in the beginning. Our work on joint return distribution lays foundations for such future works. Our work only use the expectation of total returns from different sources to make decision, leaving the more complex algorithms to future work. }
%\textcolor{red}{ With our method, we can build rich, implicit model of the environment, as well as being compatible with value-based RL algorithms. 

%In this work, we propose the MD3QN, a distributional RL algorithm that learns a high-dimensional joint distribution for multiple sources of reward by temporal difference loss. The effectiveness of our method can be verified on pixel-input environments on both the quality of modeled joint distribution on hybrid reward sources, and the final performance on policy optimization. Building a reliable framework to learn a high-dimensional joint distribution model in RL has significant importance for modeling highly informative information in value network. In the future, we will further explore the direction on extending the value network to capture more information like state distributions, and MD3QN proposed by this paper can provide fundamental supports in this direction. 

==> src/5-method.tex <==
\section{Hybrid Reward Distributional Reinforcement Learning}

In this paper, we propose to capture the correlated randomness from multiple reward sources, forcing the agent to gain more knowledge about the environment and learn better representations. Specifically, we consider the joint distribution of returns from different reward sources. 
First, we introduce the joint distributional bellman operator and establish its convergence. We correct the misunderstanding in existing work~\citep{bellemare2017distributional,nguyen2020distributional}, that we must use the same metric for proving convergence and as training loss. We illustrate that, once the convergence of Bellman operator is proved under certain metric, we can use other metrics than the metric for proving convergence, as training loss to approximate the Bellman operator. 
Second, we introduce an empirical algorithm, which approximates Bellman operator through stochastic optimization with deep neural networks. Inspired by MMDQN~\citep{nguyen2020distributional}, we introduce a temporal difference loss based on Maximum Mean Discrepancy over joint return distributions.
Finally, we give full implementation details of our method, including network architectures and algorithms \sout{for loss computation}. % In order to adapt to multiple reward sources with different reward scale, we also introduce re-weighted norm with adaptive weight for gaussian kernels in the MMD loss to balance between rewards from different sources.

%\textcolor{blue}{In this paper, we consider the joint return distribution under the hybrid reward setting. First, we introduce the joint distributional bellman operator and establish its convergence. To approximate such operator through stochastic optimization in practical algorithm with deep neural networks, we then introduce a temporal difference loss based on Maximum Mean Discrepancy over joint return distributions, as inspired by \cite{}. Finally we give full implementation details of our method, including network architectures and loss computations. }

%\textcolor{red}{Both the theoretical and algorithmic parts of our method can be seen as extensions of existing theoretical and algorithmic works on 1-dimension to K-dimension. It is worth mentioning that such extension is non-trivial, in that we fix some issues and make some adaptations to K-dimension. We find the 1-dimensional contraction proof in \cite{C51} skip some steps, making it hard to follow, therefore we give a more detailed contraction proof under the joint distribution setting. While the original algorithm in 1-dimension takes use of deterministic samples from return distribution, we propose to estimate stochastic samples with more flexibility to approximate the whole return distribution as the number of samples approach infinite. In order to deal with different scale of reward from hybrid sources, we also introduce re-weighted norm for gaussian kernels in the MMD loss. }


%We first define the hybird-source return as a K-dimensional random variable, and introduce Wasserstein metric $Wp$ the joint distribution and  on the settings and establish the convergence of the joint distributional bellman operator. 


%In this section, we firstly focus on the settings and convergence analysis for learning the joint value distribution of hybrid-source return. We prove that iteratively \textcolor{blue}{applying} %adapting by 
%joint distributional Bellman operator will make the estimation converge to the ground truth value distribution. 
%We then introduce a temporal difference error based on metric over joint value distribution, and explain why optimizing the loss can be approximated as applying joint distributional Bellman operator. 
%Finally we give full implementation details of our method, including network architectures and loss computations. 


\subsection{Definitions and Settings}

%We define $\vec{Z}^\pi(s,a)$ as
We consider the joint return distribution $\bm{Z}^\pi(s,a)$ under policy $\pi$ as
\begin{align}
    \bm{Z}^\pi(s,a) &\stackrel{D}{\coloneqq} \sum_{t=0}^\infty \gamma^t \bm{r}_t, \\
    \text{ where } s_0 &= s, a_0 = a, \bm{r}_t \sim R(\cdot|s_t, a_t), s_{t+1} \sim P(\cdot|s_t, a_t), a_{t+1} \sim \pi(\cdot|s_{t+1}).
\end{align}

%We can interpret $\vec{Z}^\pi(s,a)$ as the joint distribution for the discounted return of multiple source reward. 
The $i$-th dimension of $\bm{Z}^\pi(s,a)$ is the random variable for the $i$-th source of discounted return, and different dimensions in $\bm{Z}^\pi(s,a)$ can be correlated. We use $\bm{Z}: \mathcal{S} \times \mathcal{A} \rightarrow \mathcal{P}(\mathbb{R}^K)$ to denote a joint return distribution model, where $\bm{Z}(s,a) \in \mathcal{P}(\mathbb{R}^K)$ is the joint distribution predicted by the model on state action pair $(s,a)$ of future returns over multiple reward sources. The goal of our algorithm is to let model $\bm{Z}$ to be as close to $\bm{Z}^\pi$ as possible in policy evaluation setting, i.e. to model the real joint return distribution. 

To measure how close two $K$-dimensional joint distributions are, we adopt Wasserstein metric $W_p$.  %If we have 
For two joint distributions $\mu, \nu \in \mathcal{P}(\mathbb{R}^K)$, the p-Wasserstein metric $W_p(\mu, \nu)$ on Euclidean distance $d$ is given by: 
\begin{equation}
    W_p(\mu, \nu) = \left(\inf_{f \in \Gamma(\mu, \nu)} \int_{\mathbb{R}^K \times \mathbb{R}^K} d(x, y)^p f(x,y) d^K x d^K y \right)^{1/p}
    %W_p(\mu, \nu) = \left(\inf_{f \in \Gamma(\mu, \nu)} \int_{\mathbb{R}^K \times \mathbb{R}^K} d(x, y)^p  \mathrm{d} f(x,y) \right)^{1/p}
\end{equation}
where $\Gamma(\mu, \nu)$ is the collection of all distributions with marginal distribution $\mu$ and $\nu$ on the first and second $K$ random variables %factors 
respectively. The Wasserstein distance can be interpreted as the minimum moving distance to move all the mass from distribution $\mu$ to distribution $\nu$. 

To measure the distance between two joint distribution models $\bm{Z}_1$ and $\bm{Z}_2$, %$W_1$ and $W_2$, 
we take the maximum Wasserstein distance over all state action pairs, formalized in the equation below. 
\begin{equation}
    %d_p(W_1, W_2) := \max_{s,a} W_p(W_1(s,a), W_2(s,a)). 
\bar{d}_p(\bm{Z}_1, \bm{Z}_2) := \max_{s,a} W_p(\bm{Z}_1(s,a), \bm{Z}_2(s,a)) 
\end{equation}
We will use $\bar{d}_p$ to establish the convergence of the joint distributional Bellman operator. 
\iffalse
\begin{lemma}
    $\bar{d}_p$ is a metric over joint return distributions.
\end{lemma}
\fi

\subsection{Convergence of Joint Distributional Bellman Operator}
%\textcolor{blue}{We extend the theoretical results on distributional bellman operator from 1-dimension distribution in C51, to high-dimensional distribution in our case. It is worth mentioning that it is non-trivial to extend the theoretical results to high-dimensional distribution, where the wasserstein distance does not have nice formulation as in 1-dimensional case. Detailed proofs can be found in Appendix.  }
%The theory framework is mainly based on C51 paper \citep{bellemare2017distributional}, but our conclusion is the extension of theirs and require more work than C51. 
We define the joint distributional Bellman evaluation operator $\mathcal{T}^\pi$ as
\begin{align}
    \mathcal{T}^\pi \bm{Z}(s_t,a_t) &\stackrel{D}{\coloneqq} \bm{r}_t + \gamma \bm{Z}(s_{t+1}, a_{t+1}) \\
    \text{ where } & \bm{r}_t \sim R(\cdot|s_t,a_t), s_{t+1} \sim P(\cdot|s_t,a_t), a_{t+1} \sim \pi(\cdot|s_{t+1})
\end{align}

The below theorem shows that $\mathcal{T}^\pi$ is a $\gamma$-contraction operator on $\bar{d}_p$. % We provide detailed proof of Theorem 1 in Appendix A. 

\begin{theorem}
    For two joint distribution models $\bm{Z}_1$ and $\bm{Z}_2$, %$W_1$ and $W_2$, 
    we have
    \begin{equation}
        %d_p(\mathcal{T}^\pi W_1, \mathcal{T}^\pi W_2) \leq \gamma d_p(W_1, W_2)
        \bar{d}_p(\mathcal{T}^\pi \bm{Z}_1, \mathcal{T}^\pi \bm{Z}_2) \leq \gamma \bar{d}_p(\bm{Z}_1, \bm{Z}_2).
    \end{equation}
\end{theorem}
We consider the following scenario: initially we have a joint distribution model $\bm{Z}_0: \mathcal{S} \times \mathcal{A} \rightarrow \mathcal{P}(\mathbb{R}^K)$, and iteratively adapt the model by $\bm{Z}_{i+1} = \mathcal{T}^\pi \bm{Z}_i $. 
According to Banach's fixed point theorem, operator $\mathcal{T}^\pi$ has a unique fixed point, which is $\bm{Z}^\pi$ by definition. 
%Since $\bm{Z}^\pi$ is the fix point of operator $\mathcal{T}^\pi$, 
The distance between $\bm{Z}_i$ and $\bm{Z}^\pi$ decays as $i$ increases. We have the following proposition: 
\begin{proposition}
    If $\bm{Z}_{i+1} = \mathcal{T}^\pi \bm{Z}_i $, then as $i \rightarrow \infty$, $\bm{Z}_i \rightarrow \bm{Z}^\pi$. 
\end{proposition}

We also provide contraction proof on expectation of the optimality operator.
%%%%%% \blue{Please check here}
The joint distributional Bellman optimality operator $\mathcal{T}$ is defined as
\begin{align}
    \mathcal{T}\bm{Z}(s_t,a_t) &\stackrel{D}{\coloneqq} \bm{r}_t + \gamma \bm{Z}(s_{t+1}, a') \label{eq-optimal-op} \\
    \text{ where } & \bm{r} \sim R(\cdot|s_t,a_t), s_{t+1} \sim P(\cdot|s_t,a_t), a'=\argmax_{a'} \mathbb{E} \sum_{k=1}^K Z_k(s_{t+1}, a') \label{eq-optimal-op-where}
\end{align}

\textcolor{red}{definition for E operator}

\begin{theorem}
    For two joint distribution models $\bm{Z}_1$ and $\bm{Z}_2$, %$W_1$ and $W_2$, 
    we have
    \begin{equation}
        %\vert \vert \mathbb{E} \mathcal{T} W_1 - \mathbb{E} \mathcal{T} W_2 \vert \vert_{\infty} \leq \gamma \vert \vert \mathbb{E}  W_1 - \mathbb{E} W_2 \vert \vert
        \vert \vert \mathbb{E} \sum_{k} (\mathcal{T} \bm{Z}_1)_k - \mathbb{E} \sum_{k} (\mathcal{T} \bm{Z}_2)_k \vert \vert_{\infty} \leq \gamma \vert \vert \mathbb{E}  \sum_{k}Z_{1,k} - \mathbb{E} \sum_{k}Z_{2,k} \vert \vert
    \end{equation}
\end{theorem}
%\textcolor{red}{redefine the expectation here! Should be sum over all sub-returns. }
where $Z_{\cdot,k}$ represents the marginal distribution for the $k$-th source-specific return.
%%%%%%

\begin{proposition}
    If $\bm{Z}_{i+1} = \mathcal{T} \bm{Z}_i $, then as $i \rightarrow \infty$, $\mathbb{E}[\sum_{k=1}^{K} Z_{i,k}] \rightarrow Q^*$%\mathbb{E}[\sum_{k=1}^{K} Z^{*}_{i,k}]$. 
\end{proposition}

The proposition 2 can be interpreted as following: as we iteratively apply the joint distributional Bellman optimality operator, the expected total return of the joint distribution predicted by the model $Z_i$ will converge to optimal value function. We refer the readers to the appendix for details proofs for all the lemmas, theorems, and propositions.


%There is a common misunderstanding in existing work that it is necessary to use the same metric to prove convergence and as training loss~\citep{bellemare2017distributional, nguyen2020distributional}. However, we argue that, convergence is the property of the operator itself, regardless of the metric. If the operator is proved to be contraction under one metric, then applying the operator iteratively will lead to convergence to a fixed point. In contrast, training loss is used to "apply" the operator. In fact, we can use any loss, as long as we can guarantee the distribution and its Bellman target are identical when the loss is minimized. 
%For example, in C51~\citep{bellemare2017distributional}, the Cramer distance is used implicitly in the projection step, and the projected operator is proved to be contraction under cramer distance. Then, we can apply this projected operator with KL-divergence, since KL-divengence is minimized if and only if two distributions are identical. \textcolor{red}{maybe we need to week the claim}
\textcolor{blue}{There is a common misunderstanding in existing works that we must use the same metric to prove convergence and as training loss~\citep{bellemare2017distributional, nguyen2020distributional}. We clarify that the metric for proving convergence and the metric for training loss play different roles, and are not necessarily the same metric. 
For example, Cramer distance is used to prove the contraction property of the projected Bellman operator in C51~\citep{pmlr-v84-rowland18a}. The contraction property leads to the convergence property. KL-divergence is used to approximate the projected operator in C51~\citep{bellemare2017distributional}. With infinite sampled transitions and expressive value networks, we can approximate the projected operator exactly when the KL-divergence is minimized. }


\subsection{Optimizing MMD as approximation for Bellman Operater}

%\textcolor{blue}{1. We extend existing distribution RL algorithm to high-dimensional? or we approximate the joint distributional bellman operator with xxx loss? 2. C51 is not easy to scale to high-dimensional. Sample-based method is much better.3. approximate continuous distribution with samples. logic is not clear yet. Try to figure out a good logic tomorrow. }

In practical algorithms, the joint distributional model $\bm{Z}_i$ is represented by deep neural network $\bm{Z}(s,a;\theta_{i})$ with parameter $\theta_i$. We cannot directly apply the Bellman operator as in tabular case. Moreover, we only have sampled transitions, rather the the environment dynamics model $P$. It is desirable to choose a loss that is compatible with stochastic optimization, as an approximation for Bellman operator. 

%In practical algorithms, the joint distribution model $\bm{Z}_i$ is approximated by the target network. We suppose for each iteration $i$, $\bm{Z}_{i}(s,a) := \bm{Z}(s,a,z;\theta_{i})$ where $\theta_{i}$ parameterizes the joint distribution model $\bm{Z}_{i}$ and $z \sim p(z)$ is noise parameter with distribution $p(z)$. Our objective is to find the optimal parameter $\theta_{i+1}$ to make the online network $\bm{Z}_{i+1}=\bm{Z}(s,a,z;\theta_{i+1})$ match the joint distribution $\mathcal{T}^\pi \bm{Z}_i$ in policy evaluation setting, and match joint distribution $\mathcal{T} \bm{Z}_i$ in policy optimization setting. In the following discussion, we focus on policy optimization setting, and analysis for policy evaluation setting is similar. 

We achieve this by minimizing the Maximum Mean Discrepancy (MMD) between joint distribution $\bm{Z}_{i+1}$ and $\mathcal{T} \bm{Z}_i$, which is defined as the equation below. 
\begin{equation}
\label{eq-mmd-definition}
    \text{MMD}^2(p, q; k) = \mathbb{E}_{x, x' \sim p}k(x, x') - 2\mathbb{E}_{x\sim p, y \sim q}k(x, y) + \mathbb{E}_{y, y' \sim q} k(y, y'),
\end{equation}
where $k(\cdot, \cdot)$ is some kernel function and MMD is defined upon $k$, and each pair of random variable in $(x, x'), (x, y), (y, y')$ are independent. In our scenario, we use $\text{MMD}^2(\bm{Z}_{i+1}, \mathcal{T} \bm{Z}_i)$ as the temporal difference loss. 
\textcolor{blue}{The reason why we choose MMD as the objective function is that MMD is both a metric on distribution and} \textcolor{red}{can be optimized with sampled transitions}. 
%\textcolor{blue}{As we can see from the definition, MMD is easy to optimize with sampled transitions.}
%\textcolor{blue}{One may wonder if it is necessary to prove the contraction of Bellman operator under MMD, as in previous work on 1-dimentional distributional RL with MMD\cite{MMD-DQN}. However, we argue that, if the operator is proved to be contraction under one metric, then iterative applying the operator will converge. To ``apply" the operator, we just need a loss that is a metric, so that when the loss is zero we can guarantee that the two distribution is identical.} 
%The reason why we choose MMD as the objective function is that MMD is both a metric on distribution and easy to optimize. 
The original paper of MMD \citep{gretton2012kernel} proves that MMD is a metric on distribution when kernel $k$ is characteristic, from which we can prove that
\begin{equation}
    \bm{Z}_{i+1} = \mathcal{T} \bm{Z}_i \iff \forall (s,a) \in \mathcal{S} \times \mathcal{A}, \text{MMD}^2(\bm{Z}_{i+1}(s,a),\mathcal{T} \bm{Z}_i(s,a);k) = 0,
\end{equation}
when the kernel $k$ is characteristic. If the MMD metric is optimized to zero and appropriate kernel is selected, 
%we have the exact value adaptation of 
$Z_{i+1}$ is the result of exactly applying the joint distributional Bellman operator. 
We refer reader to Section 3.4 where we detail how we choose of our kernel function. % $k(x, y) = \exp(-\|x - y\|_2^2 / h)$

\textcolor{blue}{MMD is defined in terms of expectation. In practice, we calculate loss based on samples from distribution to get an unbiased estimation of MMD. Here, we use stochastic samples rather than deterministic samples as in MMDQN, to capture the rich information of joint return distributions. To be specific, we model the return distribution as $\bm{Z}(s,a,z;\theta_{i})$ where $\theta_{i}$ parameterizes the joint distribution model $\bm{Z}_{i}$ and $z \sim p(z)$ is noise parameter with distribution $p(z)$. By sampling the noise $z$, we can get stochastic samples $x = \bm{Z}(s,a,z;\theta_{i})$ from distribution $\bm{Z}_i$. With stochastic samples, we can approximate the expected MMD loss then the number of samples approach infinity. Algorithm 1 give details on how to computes the gradient of the MMD metric based on sampled data. 
}

\textcolor{red}{replace this paragraph by the analysis of unbiased estimation}

\iffalse
For the optimization of MMD metric, 
since the third term in equation \ref{eq-mmd-definition} has no gradient to $p$, we have the gradient form of MMD metric with respect to parameter $\theta_{i+1}$ as follows: 
\begin{align}
    &\ \ \ \ \nabla_{\theta_{i+1}}\text{MMD}^2(\bm{Z}_{i+1}(s,a), \mathcal{T} \bm{Z}_i(s,a); k) \nonumber \\
    &= \nabla_{\theta_{i+1}}\left[\mathbb{E}_{x, x' \sim \bm{Z}_{i+1}(s,a)}k(x, x') - 2\mathbb{E}_{x\sim \bm{Z}_{i+1}(s,a), y \sim \mathcal{T} \bm{Z}_i(s,a)}k(x, y)\right] \label{eq-gradient-mmd}
\end{align}

The benefits of using MMD is that, in the above gradient form both the first and the second expectation term can be unbiasedly estimated with batched data. We detail this claim in the next paragraph. 

Suppose we are given a transition sample $(s,a,r,s',a')$ where $a'$ maximize the expected total return same as equation \ref{eq-optimal-op-where}. We sample $x_{1:N} \stackrel{i.i.d.}{\sim} \bm{Z}_{i+1}(s,a)$ and $x_{1:N}^{target} \stackrel{i.i.d.}{\sim} \bm{Z}_i(s',a')$, and compute $y_{1:N}$ by $y_i= r + \gamma x_{i}^{target}$ for $i=1,2,\cdots,N$. It is clear that $k(x_i, x_j)$ forms the sample in the first term when $i \neq j$, since $x_i, x_j$ are independently sampled. Also, $y_{1:N}$ form the samples from distribution $\mathcal{T} \bm{Z}_i(s,a)$ and $k(x_i, y_j)$ forms the sample in the second term of equation \ref{eq-gradient-mmd} for all $(i,j)$. In summary, $x_{1:N}$ and $y_{1:N}$ can be used to give an unbiased gradient estimate for equation \ref{eq-gradient-mmd}.

% \blue{Compared to previous metric, show why MMD is easy to optimize}
Algorithm 1 wraps up discussions above and shows how HRDRL computes the gradient of the MMD metric based on sample data. 
\fi

\begin{algorithm}[]
\caption{Optimization of MMD metric by transition samples}\label{algorithm-1}
\begin{algorithmic}[1]
\STATEx \textbf{Require: } Number of samples $N$, kernel $k$, discount factor $\gamma \in (0, 1)$, policy $\pi$ if performing policy evaluation
\STATEx \textbf{Require: } Joint distribution network $\bm{Z}(s,a,z;\theta)$
\STATEx \textbf{Input: } Transition sample $(s, a, r, s')$
\STATEx \textbf{Input: } Online network parameter $\theta$, target network parameter $\theta'$
\STATEx \textbf{Output: } Gradient estimation of MMD with respect to $\theta$
\IF {Policy evalution setting}
    \STATE $a' \sim \pi(\cdot|s')$
\ELSE
    \STATE $a' \leftarrow \argmax_{a'} \sum_{k=1}^K\frac{1}{N}\sum_{i=1}^N \bm{Z}(s', a',z_i;\theta')_k $, where $z_{1:N} \sim p(z)$. 
\ENDIF
\STATE $x_i \leftarrow \bm{Z}(s,a,z_i;\theta)$, where $z_i \sim p(z)$, for every $1 \leq i \leq N$
\STATE $x_i^{target} \leftarrow \bm{Z}(s,a,z_i^{target};\theta')$, where $z_i^{target} \sim p(z)$, for every $1 \leq i \leq N$
\STATE $y_i \leftarrow r + \gamma x_i^{target}$, for every $1 \leq i \leq N$
\STATE $\text{MMD}^2 \leftarrow \sum_{1 \leq i \leq N} \sum_{1 \leq j \leq N, j \neq i} \left[ k(x_i, x_j) - 2k(x_i, y_j)  + k(y_i, y_j)\right]$
\STATE \textbf{return} $\nabla_{\theta} \text{MMD}^2$

\end{algorithmic}
\end{algorithm}

\subsection{Network Architecture and Implementation Details}

We illustrate our network architecture in Figure \ref{img-network-architecture}. For a given state-action pair $(s,a)$, we use the Nature DQN network to compute the embedding of state $s$ with all possible actions, and select the embedding corresponding to action $a$ to get the embedding $c(s,a)$. We use gaussian distribution $N(0,1)$ as the noise distribution $p(z)$, and multple samples of random noise $z \sim p(z)$ is concatenated to embedding $c(s,a)$, then feed forward with MLP to output the samples of $\bm{Z}(s,a)$. The output of neural network is $K$-dimensional vector, representing one sample of $K$ hybrid-source return.

\textcolor{red}{replace network architecture part, and graph}
\iffalse
\begin{figure}
  \centering
  \includegraphics[width=12cm]{files/hrmmd.pdf}
  \caption{Network architecture for joint distribution model. }
  \label{img-network-architecture}
\end{figure}
\fi

We follow the kernel selection in MMDQN \citep{nguyen2020distributional} and apply the gaussian kernel function with mixed bandwidth. \textcolor{red}{characteristic kernel}

% \textcolor{red}{
%Here we make our second modification, to adapt to the different reward scale under hybrid reward setting. However, the reward scale could be different for different reward sources. By using the original L2 norm in gaussian kernel, we may ignore the changes for reward sources with small scales. To deal with such problem, we adopt a re-weighted L2 norm rather than original L2 norm in 1-dimensional setting, which can be expressed as follows: }
% \textcolor{red}{Change the norm to re-weighted norm here!!!}

\begin{align}
    k(x, x') &= \sum_{i=1}^{B} k_{b_i}(x,x') \\
    \text{ where } k_b(x, x') &= e^{-\frac{\|x - x'\|_2^2}{b}}
\end{align}

It is worth noting that when the bandwidth $b_i > 0$ is too small or too large, the kernel function converge to 0 or 1 respectively and the gradient for MMD converge to zero. We choose the value of bandwidth $b_i$ with diverse range, specifically $b_i = 2^{i-2}$ for each $1 \leq i \leq 8$, to make sure that all scales of reward don't suffer from gradient vanishing. 

\iffalse
\textcolor{red}{We also keep an exponential moving average of expectation of each dimension in TD target, $r_k + \gamma \mathbb{E}[Z_{i,k}]$, and use those statistics to reweight L2 norm. 
This trick also enables us to deal with no-reward clipping setting in Atari Games. 
}

\fi
